Adaptive Bitrate Streaming Over Cellular Networks: Rate Adaptation and Data Savings Strategies

Adaptive bitrate streaming (ABR) has become thede factotechnique for videostreaming over the Internet. Despite a flurry of techniques, achieving high quality ABRstreaming over cellular networks remains a tremendous challenge. First, the design ofan ABR scheme needs to balance conflicting Quality of Experience (QoE) metrics suchas video quality, quality changes, stalls and startup performance, which is even harderunder highly dynamic bandwidth in cellular network. Second, streaming providers havebeen moving towards using Variable Bitrate (VBR) encodings for the video content,which introduces new challenges for ABR streaming, whose nature and implicationsare little understood. Third, mobile video streaming consumes a lot of data. Althoughmany video and network providers currently offer data saving options, the existingpractices are suboptimal in QoE and resource usage. Last, when the audio and videotracks are stored separately, video and audio rate adaptation needs to be dynamicallycoordinated to achieve good overall streaming experience, which presents interestingchallenges while, somewhat surprisingly, has received little attention by the researchcommunity. In this dissertation, we tackle each of the above four challenges.

==> Audio/abstract.tex <==

%\begin{abstract}
Adaptive bitrate (ABR) streaming is the predominant approach for video streaming over the Internet.
When the audio and video tracks are stored separately (i.e., in {\em demuxed} mode), the client needs to dynamically determine which audio and which video track to select for each chunk/playback position.
Somewhat surprisingly, there is very little literature on how to best mesh together audio and
video adaptation in ABR streaming. In this paper, we first examine the state of the art in the handling of demuxed audio and video tracks in predominant ABR protocols (DASH and HLS), as well as in real ABR client implementations in three popular players covering both browsers and mobile platforms. Combining experimental insights with code analysis, we shed light on a number of limitations in existing practices both in the protocols and the player implementations, which can cause undesirable behaviors such as stalls, selection of potentially undesirable combinations such as very low quality video with very high quality audio, etc. Based on our gained insights, we identify the underlying root causes of these issues, and propose a number of practical design best practices and principles  whose collective adoption will help avoid these issues and  lead to better QoE. 
% \end{abstract}


%\yanyuan{ DELETE It adapts to dynamic network conditions by switching its streaming between multiple tracks/variants  encoded at different bitrates and quality levels. }


==> Audio/bing-command.tex <==

\usepackage{epsfig}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\mysection}[1]{\vspace{-.03in}\section{#1}\vspace{-.00in}}
\newcommand{\mysubsection}[1]{\vspace{-.05in}\subsection{#1}\vspace{-.01in}}
\newcommand{\mysubsubsection}[1]{\vspace{-.05in}\subsubsection{#1}\vspace{-.00in}}


\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.25\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.16\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\vspace{-.2in}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsingledash}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\vspace{-.2in}
\end{figure}
}

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.10\textwidth}
%        \setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
\vspace{-0.1in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> CAVA/abstract.tex <==
%\begin{abstract}

Adaptive Bitrate (ABR) video streaming is widely used for over-the-top (OTT) video delivery. Recently, streaming providers have been moving towards using Variable Bitrate (VBR) encodings for the video content, spurred by the potential of improving user QoE (Quality of Experience) and reducing network bandwidth requirements compared to Constant Bitrate (CBR) encodings. However VBR introduces new challenges for ABR streaming, whose nature and implications are little understood. We explore these challenges across diverse video genres, encoding technologies, and platforms. We identify distinguishing characteristics of VBR encodings that impact user QoE and should be factored in any ABR adaptation decision.  Traditional ABR adaptation strategies designed for the CBR case are not adequate for VBR. We develop novel best practice design principles to guide ABR rate adaptation for VBR encodings. As a proof of concept, we design a novel and practical control-theoretic rate adaptation scheme, CAVA (Control-theoretic Adaption for VBR-based ABR streaming), incorporating these concepts. Extensive evaluations show that CAVA substantially outperforms existing state-of-the-art adaptation techniques, validating the importance of these design principles.
%\end{abstract}


==> CAVA/bing-command.tex <==

\usepackage{epsfig}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.25\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.16\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\vspace{-.2in}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsingledash}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\vspace{-.2in}
\end{figure}
}

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.10\textwidth}
%        \setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
\vspace{-0.1in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> CAVA/roadmap.tex <==
%\subsection{Organization of the Paper}
The rest of the paper is organized as follows.
We 
%briefly review related work in \S\ref{sec:related}, and  
describe the VBR video dataset in \S\ref{sec:video-dataset}, and then describe the characteristics of VBR videos and their implication on rate adaptation in \S\ref{sec:characteristics}. Afterward, we present the design principles for streaming VBR videos  in \S\ref{sec:principles}, and the design and implementation of CAVA in \S\ref{sec:design}. Performance evaluation is presented in \S\ref{sec:perf}.  
Related work is reviewed in \S\ref{sec:related}. Last, \S\ref{sec:concl} concludes the paper and presents future directions.


==> PIA-E/abstract.tex <==
\begin{abstract}
	
Adaptive bitrate streaming (ABR) has become the \emph{de facto} technique for video streaming over the Internet. Despite a flurry of techniques, achieving high quality ABR streaming over cellular networks remains a tremendous challenge.
ABR streaming can be naturally modeled as a control problem. There has been some initial work on using PID, a widely used feedback control technique, for ABR streaming.
Existing studies, however, either use PID control directly without fully considering the special requirements of ABR streaming, leading to suboptimal results, or conclude that PID is not a suitable approach.
In this paper, we take a fresh look at PID-based control for ABR streaming. We design a framework called PIA (PID-control based ABR streaming) that strategically leverages PID control concepts and incorporates several novel strategies to account for the various requirements of ABR streaming.
We evaluate PIA using simulation based on real LTE network traces, as well as using real DASH implementation.
The results demonstrate that PIA outperforms state-of-the-art schemes in providing high average bitrate with significantly lower bitrate changes (reduction up to 40\%) and stalls (reduction up to 85\%), while incurring very small runtime overhead. We further design PIA-E (PIA Enhanced), which improves the performance of PIA in the important initial playback phase. 

\end{abstract}





==> PIA-E/bing-command.tex <==

\usepackage{epsfig}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.25\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.16\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\vspace{-.0in}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsingledash}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\vspace{-.0in}
\end{figure}
}

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.10\textwidth}
%        \setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
\vspace{-0.0in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> PIA/Kp-Ki.tex <==
\subsection{PIA: Choice of parameters} \label{subsec:kp-ki}

%\textbf{Explore the parameter space, show the range of values for $K_p$ and $K_i$ to get good performance; the choice is insensitive to chunk size, network bandwidth profile, video, startup latency, weight in QoE metric, startup latency. fix buffer size to 60 s (to accommodate chunk size of 8 seconds). Provide insights why.


%The Kp and Ki are very resilient for good performance in QoE.  PID parameter will not change if we change the video bitrate sets.

%We use systematic search to find the proper zone for  the combination of $K_p$ and $K_i$. We adopt the QoE metric \cite{yin2015control} for the evaluation of performance.

%The proportional and integral parameters, $K_p$ and $K_i$, are two important parameters of PIA.

%$K_p$ and $K_i$ for PIA
Following the methodology outlined in Section~\ref{subsec:PIA-tuning}, we first tune $K_p$ and $K_i$, and then tune $\beta$ for PIA.
%We next investigate how to tune $K_p$ and $K_i$ in PIA and
One question is whether there exist a set of $K_p$ and $K_i$ values that work well in a wide range of settings.
This is an important issue related to the practicality of PIA because if the choice of $K_p$ and $K_i$ were sensitive to the settings,
then tuning them for different settings would require more efforts.
 %and one needs to tune $K_p$ and $K_i$ depend on the settings, then the tuning efforts would be prohibitive. \feng{I would not say ``prohibitive''. Just say there's more overhead of turning the paras.}
 While as described earlier, the quality of experience (QoE) is affected by three metrics (average video bitrate, the amount of bitrate changes and rebuffering) jointly, comparing the QoE under different choices of $K_p$ and $K_i$ is much simpler when using a single combined metric. There is no consensus on such a metric. One approach is using a weighted sum of the three metrics as in~\cite{yin2015control}.
 %Following the approach in~\cite{yin2015control}, we use a weighted sum of the three metrics as QoE.
 Specifically, for a video of $N$ chunks,
\begin{eqnarray}
\label{eq:qoe}
\text{QoE}=\sum_{t=1}^{N}R_t -\mu \sum_{t=1}^{N-1}\left|R_{t+1}-R_t\right| - \lambda \sum_{t=1}^{N} S_t.
\end{eqnarray}
%\feng{$\mu$ has already been used in Equ~\ref{eq:lms}. Use a different symbol.}
where
%$N$ is the number of chunks in a video,
$R_t$ is the bitrate of the $t$-th chunk and $S_t$ is the amount of stalls for the $t$-th chunk, and $\mu$ and $\lambda$ are weights that represent respectively the importance of the middle and last terms (i.e., bitrate changes and rebuffering) relative to the first term (i.e., average bitrate) in the sum.
%\feng{The middle term corresponds to the penalty from bitrate switches.}
There is no well agreed upon settings for $\mu$ and $\lambda$; we vary $\mu$ and $\lambda$ to multiple values for sensitivity test.


\begin{figure}[ht]
 \centering
    \subfigure[Heatmap.\label{subfig-1:heatmap}]{%
      \includegraphics[width=0.44\textwidth]{PIA/figs/heatmap.pdf}
    }
    \subfigure[Histogram of ``heat" values.\label{subfig-2:heatmap_dist}]{%
      \includegraphics[width=0.44\textwidth]{PIA/figs/heatmap_hist.pdf}
    }
    \caption{Region of $K_p$ and $K_i$ and the corresponding ``heat" values in one setting (bitrate level set $\mathcal R_3$, chunk size 2s, video length 20 min,  startup latency 10s, $\mu=1$, $\lambda=8.5$ (when bitrate is represented in the unit of Mbps)).}
    \label{fig:region-kpki}
\end{figure}

The trace-driven simulation allows us to conveniently consider a wide range of settings by varying video bitrate level set, video length, chunk size, startup latency, and $\mu$ and $\lambda$ in (\ref{eq:qoe}). Specifically, the video bitrate level set is either $\mathcal R_1$, $\mathcal R_2$, or $\mathcal R_3$, video length is 5, 10 or 20 minutes, chunk size is 2, 4 or 8 s, startup latency is 5, 10 or 15 s, and $\mu$ is 1 or 2, and $\lambda$ is the maximum bitrate level of a video (e.g., 3 Mbps in $\mathcal R_1$) or twice as much. The choice of of $\mu$ and $\lambda$ is based on the settings in~\cite{yin2015control}. In each setting (i.e., after fixing the above parameters), we consider each of the 50 network bandwidth traces individually.
%\feng{The following sentence does not parse. Rewrite it.}
For the $k$-th network trace, we vary the values of $K_p$ and $K_i$ in a large range to find the pair of $K_p$ and $K_i$ that maximizes the QoE (note that as described in Section~\ref{sec:PID}, we only consider valid combinations of $K_p$ and $K_i$ values, i.e., those so that the damping ratio is in $[0.6,0.8]$).
Once the maximum QoE, denoted as $Q^*_k$, is determined, the QoE under each valid ($K_p$, $K_i$) pair is compared to $Q^*_k$ to see whether it is within $90\%$ of $Q^*_k$. Specifically, we define a binary function $f_k(K_p,K_i)$ for the $k$-th network bandwidth trace, where $f_k(K_p,K_i)=1$ if the resulting QoE under $K_p$ and $K_i$ is within $90\%$ of $Q^*_k$,
%%\feng{this maximum value corresponds to the maximum QoE for the $i$-th network trace (as opposed to the one across all traces), right? Explicitly say so.}
and otherwise $f_k(K_p,K_i)=0$. We then consider all the network bandwidth traces, and create a heat map with the ``heat" for each valid pair of $K_p$ and $K_i$ values as $\sum_{k} f_k(K_p,K_i)$. Clearly, a larger ``heat" value for a $K_p$ and $K_i$ pair means that it leads to good performance for more network bandwidth traces. Fig.~\ref{subfig-1:heatmap} shows an example heat map for one set of parameters (described in the caption of the figure).
% \feng{We call the heatmap an ``example'' because it corresponds to one parameter set, right? If so say that.}
The black region represents invalid $K_p$ and $K_i$ pairs (i.e., those causing the damping ratio out of $[0.6,0.8]$). For the valid $K_p$ and $K_i$ pairs, the ``heat" value varies, with the highest values in the bottom left region, marked by the rectangle. Fig.~\ref{subfig-2:heatmap_dist} is  the histogram of the ``heat" values in
the rectangle area (excluding those corresponding to invalid $K_p$ and $K_i$ pairs). It shows that majority of the values are close to 50 (i.e., the maximum ``heat"), indicating that the valid $K_p$ and $K_i$ pairs marked by the rectangle provide good performance across almost all network traces.
%under common network conditions.
%\feng{Remind readers what are ``90\%'' and ''95\%'' in the figure -- they are the cut off thresholds of the binary function $f_i$.}



We repeat the above procedure for all the settings, and find the following region of $K_p$ and $K_i$ values leads to good performance for all the settings
\begin{equation}
\begin{split}
{K_p} \in \left[ {1 \times {{10}^{ - 3}}, 14 \times {{10}^{ - 3}}} \right]\\
{K_i} \in \left[ {1 \times {{10}^{ - 5}}, 6 \times {{10}^{ - 5}}} \right]\\
\text{s.t.}\,\,\zeta \left( {{K_p},{K_i}} \right) \in \left[0.6, 0.8\right].
\end{split}
\label{eq:good-Kp-Ki}
\end{equation}
Specifically, under the above range of values, the average ``heat" for the different settings varies from 31 to 50, and the standard deviation varies from 0.25 to 3.45.
The results in the rest of the paper use $K_p=8.8\times 10^{-3}$, approximately the middle of the range of $K_p$ in (\ref{eq:good-Kp-Ki}), and $K_i=3.6\times10^{-5}$ so that the damping ratio is ${1}/\sqrt{2}$, a widely recommended value for damping ratio~\cite{ogata2010modern,McClamroch80:State-Models}.
%%The damping ratio 0.707 is generally considered to correspond to the "fastest" response; it represents a compromise between overshoot the rise time.


The finding that a small set of $K_p$ and $K_i$ values work well under a wide range of settings is encouraging. Comparing video characteristics (chunk size, bitrate levels) and network conditions, network conditions represent the environment in which PIA operates, and hence play a more important role in determining $K_p$ and $K_i$ values. Considering that the network traces were collected under a wide range of settings and that they exhibit significantly different characteristics (see Fig.~\ref{fig:trace-charact}), our results show that $K_p$ and $K_i$ can be tuned to accommodate the large variations among individual traces. Fundamentally, this indicates that we can find a range of $K_p$ and $K_i$ values to make the system capable of dealing with the rapid bandwidth variations, which are
known to be one of the predominant characteristics of cellular networks, despite the differences across individual network conditions.



\input{PIA/explore-beta}


==> PIA/PIA-enhanced.tex <==
\subsection{PIA performance enhancing techniques} \label{subsec:PID-enhanced}

Based on the core component of PIA, we now add three domain-specific enhancements to further improve the robustness and adaptiveness for ABR streaming.

\noindent{\textbf{Accelerating initial ramp-up.}}  At the beginning of the video play, the buffer level $x_t$ can be much smaller than the target buffer level $x_r$. In this case, observe from (\ref{eq:PID-video-streaming}) that $u_t$ will be large, which will result in low video bitrate, $R_t$. To address this issue, we include a setpoint weighting parameter~\cite{astrom08:feedback},  $\beta \in (0,1]$, into the control policy as
\vspace{-.05in}
\begin{eqnarray}
%u_t &=& {K_p}({\beta x_r} - x_t) + {K_i}\int\limits_0^t {(x_r - x_\tau)d\tau} \nonumber \\
u_t = {K_p}({\beta x_r} - x_t) + {K_i}\int_0^t {(x_r - x_\tau)d\tau} + \textbf{1}(x_t - \Delta).\
\label{eq:PID-video-streaming-improved}
\end{eqnarray}
Note that $\beta$ is only included in the proportional term; it does not affect the steady-state behavior of the control system~\cite{astrom08:feedback}. When $\beta=1$, the above control policy reduces to (\ref{eq:PID-video-streaming}). When $\beta < 1$, it can lead to smaller $u_t$, and hence faster initial ramp-up in video bitrate.
 However, very small $\beta$ can lead to aggressive choice of video bitrate, and hence rebuffering at the beginning of the playback. We explore how to set $\beta$ in Section~\ref{subsec:kp-ki}.
%Note that $\beta$ only affects the transient stage and does not affect the steady-state behavior of the control system since
The control function corresponding to the above control policy is
\begin{eqnarray}
T(s) = \frac{x(s)}{x_r(s)} = \frac{\beta K_ps + K_i}{s^2 + K_p s + K_i}\,. \label{eq:Ts-with-beta}
\end{eqnarray}
Therefore, both damping ratio and natural frequency remain the same as before.
%Last, $\beta$ only affects the transient stage and does not affect the steady-state behavior of the control system~\cite{astrom08:feedback}.
%\feng{From your description, $\beta$ seems need to be adjusted dynamically throughout the video playback (a small value at the beginning then a large one later.}

\smallskip
\noindent{\textbf{Minimizing bitrate fluctuations.}} The simple choice of $R_t$ in (\ref{eq:pid_bitrate}) mainly tracks the network bandwidth and does not take into account the smoothness of the video; it may lead to frequent and/or abrupt bitrate changes.
%We develop a regularized least squares formulation to address the above issue. Specifically, the formulation considers both video bitrate and the changes in video bitrate so that it can achieve a balance of both. It minimizes the following objective function,
To address the above issue, we develop a regularized least squares (LS) formulation that considers both video bitrate and the changes in video bitrate to achieve a balance between both of these metrics.
%for a selected $u_t$,  the improved version determines the bitrate of the $t$-th chunk, $R_t$, by solving a regularized least squares problem.
Specifically, it minimizes the following objective function
\vspace{-.05in}
\begin{eqnarray}
\label{eq:lms}
J({R_t}) = \left(\sum\limits_{k = t}^{t + L} \left({u_k}{R_t} - \hat C_{k}\right)^2\right) + \eta \left(R_t - R_{t - 1}\right)^2,
\end{eqnarray}
where $R_{t-1}$ is the video bitrate for chunk $t-1$ (i.e., the previous chunk), $u_k$ is the controller output for the $k$-th chunk (based on the decision of using $R_t$ as the bitrate), $\hat C_k$ is the estimated link bandwidth for the $k$-th chunk, and $\eta$ is the weight factor for bitrate changes.
To reduce the number of video bitrate changes, the formulation assumes that the bitrate for the next $L$ chunks to be the same, all equal to $R_t$. In (\ref{eq:lms}), the first term aims to minimize the difference between $u_k R_t$ and the estimated network bandwidth $\hat C_{k}$ (so as to
maximize $R_t$ under the bandwidth constraint and selected $u_k$);
%%maximize $R_t$ (i.e., by matching $u_t R_t$ to the estimated network bandwidth as much as possible);
the second term aims to minimize the bitrate changes compared to $R_{t-1}$;
%The weighted sum balances both metrics.
the weight factor $\eta$ can be set to reflect the relative importance of these two terms. We use $\eta=1$ (i.e., equal importance) in the rest of the paper.

The above formulation takes into account both the history (i.e., $R_{t-1}$) and future time slots (through a moving horizon of $L$ chunks into the future). In each moving horizon, the control output $u_k$ is updated according to the control policy (\ref{eq:PID-video-streaming-improved}), base on the estimated $x_k$ when choosing $R_t$ as the video bitrate. Note that the above formulation does not need to consider rebuffering explicitly because PID already maintains the playback buffer to the target level (so as to avoid rebuffering).



%Because the video bitrate is in a discrete set $\mathcal V$, which denotes the set of all possible bitrates, the solution of above problem is
Let $\mathcal R$ denote the set of all possible bitrates. The solution of (\ref{eq:lms}) is
\vspace{-.05in}
\begin{eqnarray}
%\hat R_t = \arg \mathop {\min }\limits_{\hat R_t \in \{ {R_k}\} } \{ J(R_t)\}.
R^*_t = \arg \min \limits_{R_t \in \mathcal R}  J(R_t).
\end{eqnarray}
%The rationale behind this formulation is that we utilize the PI controller to find a proper buffer filling ratio, and then optimize the video bitrate by taking the QoE factors into consideration.
We can find $R^*_t$ easily by plugging in all possible values of $R_t$, $R_t \in \mathcal R$, into (\ref{eq:lms}), and find the value that provides the minimum objective function value in (\ref{eq:lms}). For every $R_t \in \mathcal R$, obtaining $J(R_t)$ requires computation of $L$ steps. Therefore, the total computation overhead is $O(|{\mathcal R}| L)$. This is significantly lower than the complexity of $O(|{\mathcal R}|^L)$ in~\cite{yin2015control}.
%\feng{Again, discuss the tradeoff incurred by $\mu$ on bitrate fluctuation vs. playback rate}


\smallskip
\noindent{\textbf{Dealing with bitrate saturation.}} Following the control policy, $u_t$ may become negative (e.g., when the current buffer level exceeds the target buffer level).  In this case, solving (\ref{eq:lms}) will lead $R_t$ to be the minimum bitrate.
%a rational choice is to set video bitrate, $R_t$, to be the maximum value to quickly reduce the buffer level.
During this time period, if we continue using the integral term, $I_{\text{out}} = {K_i}\int_0^t {(x_r - x_\tau)d\tau}$, $u_t$ may remain negative for an extended period of time, causing $R_t$ to stay at the minimum bitrate level for an extended period of time (so called system saturation~\cite{astrom08:feedback}), and causing the buffer level to continue to grow. To deal with the above scenario, we incorporate an anti-windup technique (to deal with integral windup, i.e., integral term accumulates a significant error) for negative $u_t$, or more specifically, when $u_t \le \epsilon$, $0 <\epsilon \ll 1$.
Many anti-windup techniques have been proposed in the literature~\cite{astrom08:feedback}.
We adopt a simple technique which sets $R_t$ to the maximum value, $u_t=\epsilon$, and does not change $I_{\text{out}}$ when $u_t \le \epsilon$. This corresponds to turning off the integral control when $u_t$ is below $\epsilon$.  We set $\epsilon$ to a small positive value, $10^{-10}$, in the rest of the paper.



==> PIA/PIA-put-it-together.tex <==
\subsection{PIA parameter tuning} \label{subsec:PIA-tuning}
Three important parameters in PIA are $K_p$, $K_i$ and $\beta$, where $K_p$ and $K_i$ determine the system behavior and $\beta$ is used for faster initial ramp-up.
For a given network setting (e.g., cellular networks), since $\beta$ does not affect the steady-state behavior~\cite{astrom08:feedback}, we can first assume a fixed $\beta$ (e.g., $\beta=1$) and tune $K_p$ and $K_i$ to achieve a desirable steady-state behavior (i.e., jointly maximize the three metrics in QoE). Once $K_p$ and $K_i$ are fixed, we then tune $\beta$ for the initial stage of the video playback. The values of $K_p$ and $K_i$ need to be tuned so that  the resultant system behavior is compatible with the network setting. Taking cellular networks as an example, since the bandwidth is highly dynamic, it is reasonable to tune the system so that the buffer level does not fluctuate drastically. Otherwise, the buffer can suddenly become very low, making the system vulnerable to stalls.
We describe this approach using a set of network traces from commercial cellular networks in Section~\ref{subsec:kp-ki}.

\subsection{Putting it altogether} \label{subsec:PIA-summary}


We summarize the workflow of PIA depicted in Fig.~\ref{fig:diagram}.  PIA takes the target buffer level $x_r$ and current buffer level $x_t$ as input, and computes the selected bitrate $R^*_t$, which is then fed into the Video Player Dynamics block to
update the buffer level $x_t$. PIA considers both present and past estimation errors, as well as incorporates all the three QoE metrics in
the control loop. PIA also includes an anti-windup mechanism to deal with bitrate saturation, and a setpoint weighting
technique to provide faster initial ramp-up. 



==> PIA/PIA.tex <==

%\documentclass[10pt, conference, letterpaper]{IEEEtran-v1.8}





%%%%%%%%%%%%%%%%%%%%%%%%%% COLORS
%\definecolor{brown}{cmyk}{0,0.81,1,0.60}
%\definecolor{magenta}{rgb}{0.4,0.7,0}
%\definecolor{gray}{rgb}{0.5,0.5,0.5}
%\definecolor{red}{rgb}{1,0,0}
%\definecolor{green}{rgb}{0,0.5,0}
%\definecolor{blue}{rgb}{0,0,1}

% Some very useful LaTeX packages include:
%\newcommand{\fengtext}[1]{{\color{red}#1}}

%\newcommand{\feng}[1]{{\color{red}}}
%\newcommand{\sen}[1]{{\color{blue}(SS: #1)}}
%\newcommand{\sen}[1]{{\color{blue}}}
%\newcommand{\BULLET}{\vspace{+.00in} \noindent $\bullet$ \hspace{+.00in}}

%\newcommand{\url}[1]{{#1}}

%\newcommand{\mysection}[1]{\vspace{-.03in}\section{#1}\vspace{-.00in}}
%\newcommand{\mysubsection}[1]{\vspace{-.03in}\subsection{#1}\vspace{-.00in}}
%\newcommand{\mysubsubsection}[1]{\vspace{-.00in}\subsubsection{#1}\vspace{-.00in}}


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


%\begin{document}
%

%\title{\huge A Control Theoretic Approach to  ABR Video
 % Streaming:\\A Fresh Look at PID-based Rate Adaptation}
%\chapter{PID Control for Adaptive Video Streaming over Cellular Networks}
\chapter{A Control Theoretic Approach to  ABR Video Streaming A Fresh Look at PID-based Rate Adaptation}
% make the title area
%\maketitle
%\input{PIA/abstract}

%\IEEEpeerreviewmaketitle

\input{PIA/intro}
\input{PIA/background}
\input{PIA/PIAscheme}
\input{PIA/performance}
\input{PIA/conclusion}


%\bibliographystyle{abbrv}
%\raggedright
%\bibliography{ref-bing}

%\end{document}




==> PIA/PIAscheme.tex <==
\section{Adapting PID Control for ABR Streaming} \label{sec:PID}

We propose PIA, a PID based rate adaption algorithm for ABR streaming. As shown in Fig.~\ref{fig:diagram}, it contains a PI-based core control block as well as three mechanisms to address specific requirements for ABR streaming. We first describe the core component, and then the three performance enhancing mechanisms.
%\singlefig{PIA/figs/video_PID_control}{PIA main components.}{diagram}
\begin{figure}[h]
	\centering
	\includegraphics[height=2in]{PIA/figs/video_PID_control.pdf}
	\caption{PIA main components.}
	\label{fig:diagram}
\end{figure}

\subsection{PIA core component}
The core component of PIA adjusts the standard PID control policy in equation (\ref{eq:PID}) so that the resultant closed-loop system is linear, and hence easier to control and analyze. We next define the controller output, analyze the system behavior, and  provide insights into how to choose the various parameters.

Recall the dynamic video streaming model in (\ref{eq:dynamics}), where $x_t$ is the video player buffer level at $t$, $C_t$ is the network bandwidth at time $t$, and $R_t$ is the video bitrate chosen for time $t$.
We define the controller output, $u_t$, as
%The relative buffer filling rate is
\vspace{-.05in}
\begin{equation}
\label{eq:pid_ut}
u_t = \frac{C_t}{R_t},
\end{equation}
and set the control policy as
\vspace{-.05in}
%Let the relative buffer filling rate be  the control variable $u_t$ in our system. The PID controller selects $u_t$ based on the error, i.e., the deviation of the real-time buffer level $x_t$ from the reference buffer level, $x_r$, its integral and its rate of change. Specifically,
\begin{eqnarray}
%u_t &=& {K_p}({\beta x_r} - x_t) + {K_i}\int\limits_0^t {(x_r - x_\tau)d\tau} \nonumber \\
u_t = {K_p}({x_r} - x_t) + {K_i}\int_0^t {(x_r - x_\tau)d\tau} + \textbf{1}(x_t - \Delta)
\label{eq:PID-video-streaming}
\end{eqnarray}
 where $K_p$ and $K_i$ denote, respectively, the parameters for proportional and integral control, $x_r$ denotes target buffer level, and $\Delta$ is the chunk size.
The choice of $x_r$ depends on system constraints, a point we will come back to in Section~\ref{sec:performance}.
%\feng{How do we set the target buffer level $x_r$?}

 The above control policy differs from the standard PID control policy (\ref{eq:PID}) in the last term $\textbf{1}(x_t - \Delta)$, which is a novel aspect of our design. As we shall see, it provides linearity, making the closed-loop control system easier to control and analyze. In our control policy, the parameter for derivative control $K_d=0$ (hence strictly speaking, our controller is a PI controller). This is because derivative action is sensitive to measurement noise~\cite{astrom08:feedback} and measuring network bandwidth in our context is prone to noise.
 %, which differs from
 %Note that this control policy differs from the standard PID control as in (\ref{eq:PID}) in the last term $\textbf{1}(x_t - L)$. This is a novelty in our control policy as it provides linearity as we shall see. $\beta$ is the control parameter for set point weighting, which is used to improve the transient response of the video streaming system.

Intuitively, $u_t$ defined in (\ref{eq:pid_ut}) is a unitless quantity representing the relative buffer filling rate.
%It can be larger, equal or smaller than one based on the relative values of $C_t$ and $R_t$.
With $u_t$ selected, based on (\ref{eq:pid_ut}), the player can select the corresponding bitrate as
%for the next video chunk as
\vspace{-.05in}
\begin{equation}
\label{eq:pid_bitrate}
R_t = \frac{\widetilde{C}_t}{u_t},
\vspace{-.05in}
\end{equation}
where $\widetilde{C}_t$  is the estimated link bandwidth at time $t$. Since video bitrate levels are discrete, we can choose the bitrate to be the highest that is below ${\widetilde{C}_t}/{u_t}$.
%Moving horizon estimation algorithm for computing $R_t$ is described later.
This choice of $R_t$ can increase, decrease or maintain the buffer level.
%The actual buffer level for $x_{t'}$, $t'>t$, forms as feedback to the system to update the control variable $u_{t'}$.
%In Section~\ref{subsec:PID-enhanced}, we will describe performance enhancing technique through a regularized least squared formulation.

We next analyze the system to provide insights into its behavior as well as providing guidelines in choosing parameters.
%Define \(z = \int\limits_0^t {({x_r} - x_\tau)d\tau}\) or \(\dot z = {x_r} - x_t\).
Combining equations (\ref{eq:dynamics}) and (\ref{eq:PID-video-streaming}) yields
\vspace{-.1in}
\begin{equation}
\dot x_t = u_t - \textbf{1}(x_t - \Delta) = {K_p}({x_r} - x_t) + {K_i}\int\limits_0^t (x_r - x_\tau)d\tau,
%\dot x_t = u_t - \textbf{1}(x_t - \Delta) = {K_p}({x_r} - x_t) + {K_i}z,
%\dot x_t = u_t - \textbf{1}(x_t - L) = {{K_p}({x_r} - x_t) + {K_i}z}+{K_d}{\ddot z},
%\dot x_t = u_t - \textbf{1}(x_t - L) = {{K_p}({\beta x_r} - x_t) + {K_i}z}+{K_d}{\ddot z},
\label{eq:system_eq}
\vspace{-.05in}
\end{equation}
when the video starts playback (i.e., when $t \ge \delta$). We see that it is a linear system.
Taking Laplace transform on both sides of (\ref{eq:system_eq}) yields
\vspace{-.05in}
\begin{eqnarray}
\label{eq:laplace-form}
%sx(s) &=& {K_p}(\beta {x_r}(s) - x(s)) + \frac{K_i}{s}\left({x_r}(s) - x(s)\right) \nonumber \\
sx(s) = {K_p}({x_r}(s) - x(s)) + \frac{K_i}{s}\left({x_r}(s) - x(s)\right),
%sx(s) &=& {K_p}({x_r}(s) - x(s)) + \frac{K_i}{s}\left({x_r}(s) - x(s)\right) \nonumber \\
%&+& {K_d}s({x_r}(s) - x(s)) .
\end{eqnarray}
where $s$ is a complex variable. Let $T(s)$ be the system transfer function, which describes the relationship of the input and output of a linear time-invariant system. From (\ref{eq:laplace-form}), we have
\vspace{-.05in}
\begin{eqnarray}
%T(s) = \frac{x(s)}{{x_r}(s)} = \frac{K_d{K_p}s + {K_i}}{s^2 + \frac{K_p}{K_d+1}s + \frac{K_i}{K_d+1}}.
T(s) = \frac{x(s)}{x_r(s)} = \frac{K_ps + K_i}{s^2 + K_p s + K_i}, \label{eq:Ts-1}
\end{eqnarray}
which is a second-order system. From (\ref{eq:Ts-1}), we have
\vspace{-.05in}
\begin{eqnarray}
2{\zeta}{\omega_n} = K_p, \quad {\omega_n^2} = K_i \label{eq:zeta-omega}\,,
\end{eqnarray}
where $\zeta$ and $\omega_n$ are damping ratio and natural frequency, respectively, two important properties of the system.
Solving the above two equations, we have
\vspace{-.05in}
\begin{eqnarray}
%\zeta  = \frac{K_p}{2\sqrt {K_i(K_d+1)}}, \quad \omega_n = \sqrt {\frac{K_i}{K_d+1}}.
\zeta  = \frac{K_p}{2\sqrt {K_i}}, \quad \omega_n = \sqrt {K_i}\,.
\label{eq:zeta}
\end{eqnarray}
Damping ratio represents the system's ability of reducing its oscillations. In our context, it measures how the buffer will oscillate around the target buffer level --- small damping will cause the buffer to change rapidly, while large damping will cause the buffer to change slowly.  %Empirically people have found that a damping ratio of around $0.6$ to $0.8$ yields a very good system performance~\cite{ogata2010modern}.
Natural frequency represents the frequency at which a system tends to oscillate in the absence of any driving or damping force.
Empirically it is found that $\zeta$ in the range $[0.6,0.8]$ yields a very good system performance~\cite{ogata2010modern}. As a result, $K_p$ and $K_i$  should be chosen so that $\zeta \in [0.6,0.8]$. We will discuss how to tune those parameters in Section~\ref{subsec:kp-ki}.

\input{PIA/PIA-enhanced}
\input{PIA/PIA-put-it-together}



==> PIA/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> PIA/abstract.tex <==
%\begin{abstract}
\iffalse
Adaptive bitrate streaming (ABR) has become the \emph{de facto} technique for video streaming over the Internet. Despite a flurry of techniques, achieving high quality ABR streaming over cellular networks remains a tremendous challenge. 
%This is because the adaptation needs to optimize three conflicting goals (maximizing playback bitrate, minimizing the amount of stalls and bitrate changes) over highly varying network conditions in cellular networks.
ABR streaming can be naturally modeled as a feedback control problem. There has been some initial work on using PID, a widely used feedback control technique, for ABR streaming. 
%
Existing studies, however, either use PID control directly without fully considering the special requirements of ABR streaming, leading to suboptimal results, or conclude that PID is not a suitable approach.
%
In this paper, we take a fresh look at PID-based control for ABR streaming. We design a framework called PIA that strategically leverages PID control concepts and incorporates several novel strategies to account for the various requirements of ABR streaming. 
%
We evaluate PIA using simulation based on real LTE network traces, as well as using real DASH implementation.
%from two commercial LTE networks, 
The results demonstrate that PIA outperforms state-of-the-art schemes in providing high average bitrate with significantly lower bitrate changes (reduction up to 40\%) and stalls (reduction up to 85\%), while incurring very small runtime overhead.
\fi
%Not surprisingly, PID, the most widely used feedback control technique, has been explored earlier for ABR streaming.
%Existing studies, however, either use PID control directly, not fully considering the special requirements of ABR streaming, or conclude that PID is not a suitable approach.
%Specifically, (provide some numbers).
%\end{abstract}


Adaptive bitrate streaming (ABR) has become the \emph{de facto} technique for video streaming over the Internet. Despite a flurry of techniques, achieving high quality ABR streaming over cellular networks remains a tremendous challenge.
ABR streaming can be naturally modeled as a control problem. There has been some initial work on using PID, a widely used feedback control technique, for ABR streaming.
Existing studies, however, either use PID control directly without fully considering the special requirements of ABR streaming, leading to suboptimal results, or conclude that PID is not a suitable approach.
In this work, we take a fresh look at PID-based control for ABR streaming. We design a framework called PIA (PID-control based ABR streaming) that strategically leverages PID control concepts and incorporates several novel strategies to account for the various requirements of ABR streaming.
We evaluate PIA using simulation based on real LTE network traces, as well as using real DASH implementation.
The results demonstrate that PIA outperforms state-of-the-art schemes in providing high average bitrate with significantly lower bitrate changes (reduction up to 40\%) and stalls (reduction up to 85\%), while incurring very small runtime overhead. We further design PIA-E (PIA Enhanced), which improves the performance of PIA in the important initial playback phase. 


==> PIA/background.tex <==
\section{Motivation} \label{sec:background}
%State of Art Approaches: RBA, BBA, MPC, BOLA, piStream

%\textbf{Add a table with main notation. Add a table to outline how PID developed by us differs from other approaches.}

\begin{table}
    \centering
    \begin{tabular}[h]{l|l} %\hline
 %   Symbol & Meaning   \\ \hline\hline
        $C_t$ & Network bandwidth at time $t$          \\ \hline
        $x_t$   & Buffer level at time $t$                  \\ \hline
        $x_r$     & Target buffer level         \\ \hline
	$R_t$   & Selected video bitrate for time $t$ \\ \hline
	$\Delta$ &   Video Chunk Size       \\ \hline
	$\delta$ &   Startup latency       \\ \hline
        $u_t$   & PID controller output      \\  \hline
   $K_p, K_i, K_d$ & PID controller parameters \\ \hline
        $\zeta$     & Damping ratio   \\ \hline
        $\omega_n$     & Natural frequency  \\ \hline
        $\beta$     & Setpoint weighting parameter \\ %\hline
%        $\mu$     & Bitrate Change Weight \\
%        $L$     & Look-ahead Horizon         \\	
    \end{tabular}
    \caption{Key notation.}
    \vspace{-.2in}
    \label{tab:notations}
\end{table}

%\mysubsection{Adaptive video streaming (ABR)}
%: main idea, metrics that are of interests (balancing three important metrics)
%In ABR streaming, a video clip is broken into a sequence of chunks. Each chunk contains a short interval of playback time of the content, and is made available at a variety of bitrates. When fetching a chunk, the video client selects the chunk with a suitable bitrate (and hence ABR streaming uses a client-driven approach), according to its adaptation algorithm, to react to link condition variations.

%ABR streaming has been used in many commercial systems such as Microsoft Smooth Streaming~\cite{ms-smoothstreaming}, Apple's HTTP Live Streaming (HLS)~\cite{apple-hls}, and Adobe's HTTP Dynamic Streaming (HDS)~\cite{adobe-hds}. Broadly, they can be categorized under the umbrella of Dynamic Adaptive Streaming over HTTP (DASH)~\cite{sodagar2011mpeg}.

%ABR streaming has been used in many commercial systems. 
%such as~\cite{ms-smoothstreaming,apple-hls,adobe-hds}
%Broadly, they can be categorized under the umbrella of Dynamic Adaptive Streaming over HTTP (DASH)~\cite{sodagar2011mpeg}.
%
For a satisfactory user-perceived QoE, ABR streaming needs to optimize several conflicting goals, including maximizing average playback rate, minimizing stalls (or rebuffering), and reducing sudden and frequent quality variations~\cite{dobrian2011understanding, krishnan2013video,Liu15:Deriving,ni2011flicker}. 
%Recent studies have shown that commercial ABR video players do not provide satisfactory QoE~\cite{huang2012confused,jiang2012improving,akhshabi2011experimental}, thus motivating a flurry of studies on designing better rate adaptation techniques.
%~(e.g., \cite{jiang2012improving,tian2012towards,Chen13:Scheduling,huang2014buffer,li2014probe,yin2015control,Xie15:piStream}).
We next formulate ABR streaming as a control problem and describe the motivation for our study. %For ease of reference, 
Table~\ref{tab:notations} summarizes the main notation used in this paper.
%briefly review several existing studies,


%wb, 7/21/2016, change notation for chunk size from L to \Delta since L is used later on for LMS
\subsection{ABR streaming as a control problem}
%describe video streaming can be thought of as a control problem
Deciding which bitrate level to choose can be modeled as a control problem. Specifically, let $x_t$ be the buffer level of the video player at time $t$, $C_t$ the real-time network bandwidth at time $t$, and $R_t$ the  bitrate of the video chunk that is being downloaded at time $t$. Further, let $\Delta$ denote the video chunk size (i.e., the duration of its playback time), $\delta$ denote the startup delay, i.e., how long it will take for the player to start playing. Then the player's buffer dynamics can be written as
\begin{eqnarray}
\label{eq:dynamics}
\dot x_t &=&
\begin{cases}
     \frac{C_t}{R_t},   & \text{if } t \leq \delta\\
     \frac{C_t}{R_t} - \textbf{1}(x_t - \Delta),      & \text{otherwise}
\end{cases}
\end{eqnarray}
where $\mathbf{1}(x_t - \Delta) =   1$ if  $x_t\geq \Delta$; otherwise, $\mathbf{1}(x_t - \Delta) =   0$. In other words, the playback of a chunk is only started after the entire chunk has been downloaded (a chunk contains meta data and hence the player needs to wait until the entire chunk is downloaded).

In (\ref{eq:dynamics}), $\dot x_t$ is the rate of change of the buffer at time $t$. Here, ${C_t}/{{R_t}}$ models the relative buffer filling rate.
If $C_t > R_t$, i.e., the actual network bandwidth is larger than the bitrate of the video chunk being downloaded, the buffer level will increase. Otherwise, the buffer level will be at the same level (if $C_t = R_t$) or decrease (if $C_t < R_t$).
%, i.e., the network bandwidth divided by the bitrate of the video chunk.
%and the buffer decreases only if $x_t\geq \Delta$.
%If the bitrate of the video chunk being downloaded is higher (lower) than the actual network bandwidth, the buffer level will decrease (increase).
%; and if the bit rate of the video chunk downloaded is lower than the actual link bandwidth, the buffer level will increase.

One simple control strategy is to select the video bitrate for each chunk based on the prediction of real-time link bandwidth, $\widetilde{C}_t$. Specifically, it simply chooses the highest bitrate that is less than $\widetilde{C}_t$.
%We refer to this simple strategy as \emph{Rate-based (RB)}, and use it as a baseline scheme in our evaluation in Section~\ref{sec:performance}.
This is an open-loop control (there is no feedback; the decision is based only on the current state and the model of the system).
It is not robust against network link bandwidth estimation errors. As an example, it may choose a high video bitrate if the estimated bandwidth, $\widetilde{C}_t$, is high, even if the current playback buffer level is very low. If it turns out that $\widetilde{C}_t$ is an overestimate of the actual network bandwidth, the buffer can be further drained and become empty, causing stalls.
%In addition, directly matching video bitrate to dynamic link bandwidth may lead to frequent changes in video bitrate, an undesirable behavior.
%It is therefore desirable to use closed-loop control.
Closed-loop control (or feedback control) is more effective in dealing with network link bandwidth estimation errors.



\subsection{PID control}
% As mentioned earlier, PID controller is the most widely used feedback controller in industrial control systems.
 As mentioned earlier, PID control is by far the most common way of using feedback in engineering systems.
 %A survey over eleven thousand controllers in 2002 indicates that 97\% of controllers are PID controllers~\cite{Desborough02:PID}.
 A PID controller works by continuously monitoring an ``error value" defined as the difference between the setpoint and measured process variable~\cite{astrom08:feedback}. Specifically, let $u_t$ represent the control output, and $e_t$ the error feedback at time $t$. Then
 %the input/output relation for an ideal PID controller with error feedback $e_t$ is
\begin{eqnarray}
u_t = {K_p}e_t + {K_i}\int_0^t e_\tau d\tau  + K_d \frac{de_t}{dt},
\label{eq:PID}
\end{eqnarray}
where the three parameters $K_p$, $K_i$ and $K_d$ are all non-negative, and denote the coefficients for the proportional, integral and derivative terms, respectively. As defined above, a PID controller takes account of the present, past and future values of the errors through the three terms, respectively.
Some applications may require using only one or two terms to provide the appropriate system control. This is achieved by setting the other parameters to zero. A PID controller is called a PI, PD, P or I controller in the absence of the respective control actions~\cite{astrom08:feedback}.

In the video streaming scenario, the real-time buffer level is the measured process variable, and the reference buffer level is the setpoint.
%The controller attempts to reduce the error over time by the adjustment of the control variable.
We next show that a recent state-of-the-art buffer based scheme, BBA~\cite{huang2014buffer}, can be mapped to a P-controller (though the paper does not claim any control-theoretic underpinnings).
%While a recent state-of-the-art buffer based scheme~\cite{huang2014buffer} does not claim its control-theoretic underpinning, its idea is essentially a P-controller, as we show below.
 In BBA, the video player maintains a buffer level, and empirically sets two thresholds, $\theta_\text{high} > \theta_\text{low}$.
If the buffer level is below $\theta_\text{low}$, the video player always picks the lowest bitrate, $R_{\text{min}}$; if the buffer level is above $\theta_\text{high}$, the video player picks the highest bitrate, $R_{\text{max}}$; otherwise, the video player picks the video bitrate proportionally to buffer level. The selected bitrate, $R_t$, can therefore be represented as
\begin{eqnarray*}
R_t &=&
\begin{cases}
R_{\text{min}}, & x_t < \theta_\text{low}, \\
\frac{R_{\text{max}}-R_{\text{min}}}{\theta_\text{high} - \theta_\text{low}}\left(x_t-\theta_\text{low}\right)+R_{\text{min}}, & \theta_\text{low} \le x_t \le \theta_\text{high} \\
R_{\text{max}}, & x_t > \theta_\text{high}
\end{cases}
\label{eq:bba}
\end{eqnarray*}
Comparing the above with (\ref{eq:PID}), we see that it is equivalent to a P-controller when $x_t \in [\theta_\text{low},\theta_\text{high}]$ with $K_p=\frac{R_{\text{max}}-R_{\text{min}}}{\theta_\text{high} - \theta_\text{low}}$, $K_i=0$ and $K_d=0$.


The above scheme has been tested successfully in a large-scale deployment~\cite{huang2014buffer}, indicating that a PID-type control framework has potential for ABR streaming.
On the other hand, P-controller only considers the present error (i.e., the proportional term), and ignores the other two terms. It is well known that the absence of an integral term in a system may prevent the system from reaching its target value~\cite{astrom08:feedback}. This is especially true for video streaming where inaccurate network bandwidth estimations may cause the error to accumulate over time.
%Therefore, it is important to include the integral term.
% to take account of the cumulative error to make the controller respond by applying a stronger action.
Therefore, including the integral term can potentially further improve the performance of \cite{huang2014buffer}.
PID's ability to address accumulative errors is advantageous compared to model predictive control (MPC) based approach in~\cite{yin2015control}, which does not consider accumulative errors and requires accurate network bandwidth prediction. In addition, MPC is much more computationally intensive than PID.


%We investigate using PID based control for ABR streaming in this paper, motivated by the wide adoption of PID control in practice and the success of the essentially P-Control in~\cite{huang2014buffer}.
We investigate PID-based control for ABR streaming in this paper, motivated by the widespread adoption of PID control in practice and BBA. Using PID for ABR streaming, however, has several challenges.
%
First, the goal of PID control is to maintain a target buffer level that is only indirectly related to QoE. Indeed, while maintaining the buffer at a target level can help in preventing rebuffering, it does not help with the other two metrics on playback quality and bitrate variation. Second, PID is often used in continuous time and state space, while video streaming is a discrete-time system where the decisions are made at chunk boundaries and the video bitrate levels are discrete. Finally, while PID is conceptually simple, the parameters ($K_p$, $K_i$ and $K_d$) need to be tuned carefully. Here important questions are how to choose these parameters, and to find out whether there exists a parameter set that is applicable to a wide range of settings. Some of the above challenges have been pointed out in~\cite{tian2012towards,yin2015control}, which take the position that PID is not suitable for ABR streaming. As we shall show, none of the above challenges is a fundamental hurdle for using PID-based control for ABR streaming.





==> PIA/bing-command.tex <==

\usepackage{epsfig}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.25\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.16\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\vspace{-.2in}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsingledash}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\vspace{-.2in}
\end{figure}
}

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.10\textwidth}
%        \setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
\vspace{-0.1in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> PIA/conclusion.tex <==
\section{Conclusion and Future work}
\label{sec:concl}


%%We explore harnessing control theory for rate adaptation for ABR video streaming. 
By strategically applying PID controller in an explicit and adaptive manner, PIA considerably outperforms state-of-the-art video streaming schemes
%such as BBA and MPC
in balancing the complex tradeoffs incurred by key QoE metrics, as demonstrated by extensive evaluations. PIA is also lightweight and easy to deploy.
%
We believe the same high-level principle can be applied to other multimedia applications with content quality adaptation such as live video conferencing. %and HD Voice-over-IP.
In our future work, we plan to port our implementation to mobile devices to better assess PIA's performance in the wild, and also  conduct deeper exploration of other network and streaming settings.

==> PIA/dash-results.tex <==
\subsection{Evaluation using DASH implementation}
We have implemented PIA using \texttt{dash.js} (version 2.0), a production quality open source framework~\cite{dash-js}. %It is provided by Dash Industry Forum for building video and audio players that support MPEG-DASH~\cite{dash-js}.
%
We create an emulation environment that consists of two computers: one is a Linux machine running Apache httpd as the video server and the other is a Windows machine as the client (a laptop with i7-5700HQ 3.50 GHz CPU and 16GB memory). They are connected by a 100Mbps link.
%
We then apply the Linux \texttt{tc} tool on the server side to emulate the bandwidth of the download link based on the LTE bandwidth traces we collected. We set the latency between the client and the server to 70ms as it is the average latency reported by OpenSignal's latency report. The client uses Chrome browser to run \texttt{dash.js}.
%We replace the call back function in BolaRules.js to implement PIA.
Under the \texttt{dash.js} framework, we implemented a new ABR streaming rule (about 400 LoC) to realize PIA.
%The implementation contains 356 lines of code.
%\feng{Briefly explain how you implemented PIA on dash.js. Mention the LoC if heavy engineering efforts are involved.}

\textbf{Comparing Simulation and Real Implementation Results.} We compare the results obtained from our \texttt{dash.js} implementation with those from the simulation, and confirm that the results are consistent. Specifically, for average bitrate, 90\% of the relative differences are within 6.5\%;
%For average bitrate, about 90\% of the absolute error are within 6.5\%.
for bitrate changes and and rebuffering duration, 90\% of the absolute differences are within 15 Kbps/chunk and 3 s, respectively.
%Here we use  absolute differences because the values are small.
%Kolmogorov-Smirnov test verifies that the simulation and emulation results follow the same distribution with significance level of 1\%.
Our further investigation indicates that such differences are mainly due to VBR introduced by the x.264 encoder, a setting that differs from our constant bitrate assumption in simulation. The results also indicate PIA works well for VBR videos.
%The differences
%between simulation and emulation
%are mainly because the bitrate of x.264 encoded videos for a bitrate level is not a constant value, unlike what we use in simulation.
%As the bitrate of x.264 encoded video is non-stable, we think it is the main reason for the difference between simulation and emulation.

\textbf{Runtime Overhead.}
We use a video of 903 seconds encoded using the bitrate set $\mathcal R_1$ with the chunk size of 2 s.
%The CPU utilization of running PIA is very low. It is consistently around 10\% while playing back the video (majority of the computation is for decoding). \feng{We cannot just say 10\%. We need to compare the CPU overhead of PIA vs. the CPU overhead of the default dash.js player.}
We record the CPU execution time of the ABR logic in the JavaScript code when the video is being played. The execution time of the default ABR logic in the \texttt{dash.js} player is 1.2 s for the entire 15-min video; the execution time of our PIA logic is only slightly longer (1.9 s). The results indicate PIA incurs very small runtime overhead despite its non-trivial decision process shown in Fig.~\ref{fig:diagram}.
%As default dash.js is a very simple algorithm, we think the runtime overhead of PIA is as expecting.



==> PIA/explore-beta.tex <==

%\tydubfigsingle{PIA/figs/step_response.pdf}{Step response.}{PIA/figs/avg-QoE-pid-R3.pdf}{QoE.}{Choosing $\beta$ in PIA.}{system-characteristics}

\begin{figure}[ht]
	\centering
	\subfigure[Step response.\label{subfig-1:heatmap}]{%
		\includegraphics[width=0.44\textwidth]{PIA/figs/step_response.pdf}
	}
	\subfigure[QoE.\label{subfig-2:heatmap_dist}]{%
		\includegraphics[width=0.44\textwidth]{PIA/figs/avg-QoE-pid-R3.pdf}
	}
	\caption{Choosing $\beta$ in PIA.}
	\label{fig:system-characteristics}
\end{figure}
%\vspace{-1cm}

Once $K_p$ and $K_i$ are determined, we tune $\beta$ for the initial stage of the video playback.
Specifically, we set $\beta$ to 0.01, 0.2, 0.4, 0.6, 0.8, and 1.0.
Fig.~\ref{fig:system-characteristics}(a) shows the step response of the control policy (only the results for $\beta$=0.01, 0.2 and 1 are shown for better clarity). When $\beta$ = 1, the buffer becomes full much more quickly than when $\beta$=0.2 and 0.01. This is because, as explained in Section~\ref{subsec:PID-enhanced}, lower bitrate tends to be selected when $\beta$=1, causing the buffer to fill up more quickly. To examine the three QoE metrics jointly, Fig.~\ref{fig:system-characteristics}(b) plots the QoE when playing up to the $i$-th chunk of a video of 600 chunks (the setting is the same as that for Fig.~\ref{fig:region-kpki}) when $\beta$=0.01, 0.2 or 1.
%The results for different $\beta$ values are shown in the figure.
We see that $\beta$ indeed affects the QoE for the initial playback, and $\beta$=1 leads to lower QoE compared to $\beta$=0.01 and 0.2. Further investigation reveals that $\beta$=0.01 leads to more rebuffering than $\beta$=0.2. Results in other settings show similar trends. Since rebuffering has very detrimental effects on viewing quality, we use $\beta$=0.2 in the rest of the paper.

%Fig.~\ref{fig:system-characteristics}(b) plots the QoE when playing up to the $i$-th chunk of the video (the setting is the same as that for Fig.~\ref{fig:region-kpki}), $i=1,\ldots,600$. We see that when $\beta=1.0$, the initial QoE is indeed lower than that when $\beta=0.2$ and $\beta=0.01$ (the later part of the video playback the QoEs for all values of $\beta$ are similar in ). Using $\beta=0.01$ and $\beta=0.2$ lead to similar QoE. On the other hand, using $\beta=0.01$ leads to more rebuffering (which has very detrimental effects), we therefore choose $\beta=0.2$ in the rest of the paper.

Last, the results of PIA core (i.e., without the three enhancing techniques) are also shown in Fig.~\ref{fig:system-characteristics}(b). We see that PIA core indeed leads to lower QoE compared to the full-fledged PIA, indicating the benefits of our three enhancing techniques.
 %indeed lead to better QoE (a closer look shows that they lead much higher average playback bitrate compared to PIA core, figure omitted).




==> PIA/perf-comparison.tex <==
\subsection{Performance comparison} \label{subsec:perf-comparison}

%wb, 7/28/2016, for now, let's just use three figures
%\triplefig{PIA/figs/indx-cs-2-v2-sf-3-avgbit-cdf}{}{PIA/figs/indx-cs-2-v2-sf-3-bitchange-cdf}{}{PIA/figs/indx-cs-2-v2-sf-3-rebuffer-cdf}{}
%{Performance comparison in default setting (chunk size 2 s, bitrate set $\mathcal R_2$, video length 20 mins, startup latency 10s). }{video-performance}
\begin{figure}[ht]
	\centering
	\subfigure[Step response.\label{subfig-1:heatmap}]{%
		\includegraphics[width=0.32\textwidth]{PIA/figs/indx-cs-2-v2-sf-3-avgbit-cdf.pdf}
	}
	\subfigure[QoE.\label{subfig-2:heatmap_dist}]{%
		\includegraphics[width=0.32\textwidth]{PIA/figs/indx-cs-2-v2-sf-3-bitchange-cdf.pdf}
	}
   \subfigure[QoE.\label{subfig-2:heatmap_dist}]{%
	\includegraphics[width=0.32\textwidth]{PIA/figs/indx-cs-2-v2-sf-3-rebuffer-cdf.pdf}
    }
	\caption{Performance comparison in default setting (chunk size 2 s, bitrate set $\mathcal R_2$, video length 20 mins, startup latency 10s).}
	\label{fig:video-performance}
\end{figure}


We first present the performance of PIA in the default setting, i.e., chunk size 2 s, video bitrate set $\mathcal R_2$,
video length 20 minutes,
startup latency 10 s. After that, we evaluate the impact of various parameters on the performance of PIA.
%In Section~\ref{subsec:sensitivity}, we present the sensitivity of PIA to the changes in the parameters.


%wb, 7/29/2016, old figure
%Specifically, the average bitrate of PIA is $98\%$ and $94\%$ of that of BBA and MPC, respectively, while the average amount of bitrate change is $49\%$ and $40\%$ lower, and the average amount of rebuffering is 38\% and 63\% lower than BBA and MPC, respectively.

Fig.~\ref{fig:video-performance} plots the CDF of the three QoE metrics
%(the average video bitrate, average bitrate change per chunk, and the total amount of rebuffering)
over all network bandwidth traces in the default setting.
%Fig.~\ref{fig:video-performance} presents the average video bitrate, average bitrate change per chunk, and the total amount of rebuffering for each of the network bandwidth traces. The index of the traces is sorted in increasing order of the
%average video bitrate under PIA.
The performance of four schemes, RB, BBA, MPC and PIA, are also plotted. We see that while the amount of bitrate change and rebuffering is low under RB, its average bitrate is significantly lower than those of the other schemes.
%
PIA achieves comparable average bitrate as BBA and MPC, with significantly less bitrate change and rebuffering. Specifically, the average bitrate of PIA is 98\% and 96\% of that of BBA and MPC, respectively, while the average amount of bitrate change is 49\% and 40\% lower, and the average amount of rebuffering is 68\% and 85\% lower than BBA and MPC, respectively.
%
Overall, \emph{PIA achieves the best balance among the three conflicting metrics}.
As described earlier, the inferior performance of RB is because it uses open-loop control without any feedback. The superior performance of PIA compared to BBA is because BBA implicitly uses one form of P-control (Section~\ref{sec:background}) that only takes into account present error, while PIA considers both the present and past errors.
PIA's approach of applying PID in an explicit and adaptive manner further facilitates the design and improves the performance.
The performance of MPC is sensitive to network bandwidth estimation errors~\cite{yin2015control}: it solves a discrete optimization problem in each step; when network bandwidth estimation is inaccurate, the input to the optimization problem is correspondingly inaccurate, leading to suboptimal performance.

\begin{figure}[h]
    \centering
        \includegraphics[height=2.5in]{PIA/figs/individual_cmp.pdf}
        \caption{Comparison of different schemes for one trace under the default setting (chunk size 2 s, video bitrate set $\mathcal R_2$, video length 20 minutes, startup latency 10 s).}
\label{fig:individual_cmp}
\end{figure}

To provide further insights, Fig.~\ref{fig:individual_cmp} plots the bitrate selection and the buffer level over time for BBA, MPC and PIA when using one network trace. For reference, it also plots the network bandwidth of the trace.  We clearly see that BBA has significantly more bitrate changes, and MPC tends to be more aggressive in choosing higher bitrates, which can lead to excessive rebuffering. The bitrate selection under PIA matches well with the network bandwidth without frequent bitrate changes.
%
In terms of the buffer level shown in the bottom plot in Fig.~\ref{fig:individual_cmp}, MPC is lower than that of BBA and PIA due to its aggressive choice of bitrate; the buffer level of PIA reaches steady state at around 300 s, and then stays around the target level of 60 s; the buffer level of BBA is in between that of MPC and PIA.

%Fig.~\ref{fig:LTE-metric-distribution} plots the CDF (Cumulative Distribution Function) of the average video bitrate, average bitrate change per chunk, and the total amount of rebuffering over all the traces. \textbf{Note: we only need to keep either Fig.~\ref{fig:video-performance} or Fig.~\ref{fig:LTE-metric-distribution}. Let's discuss. Fig.~\ref{fig:LTE-metric-distribution} looks cleaner.}

\smallskip
\noindent{\textbf{Impact of video length.}}
The above results are for video length of 20 mins. We can vary the ending time of the video to investigate PIA's performance for shorter videos.
%
When the ending time is larger than 5 mins (i.e., video length longer than 5 mins), we observe similar results as before; for much shorter videos, PIA has lower average bitrate compared to BBA and MPC (but still outperforms BBA and MPC on the other two metrics). This is because of the initial transient period of PIA to reach the target buffer level. Further improving the performance during the transient period is left as future work.
 %further investigation of the transient period is left as future work.



==> PIA/performance.tex <==

\section{Performance Evaluation} \label{sec:performance}

In this section, we evaluate the performance of PIA using simulation and real implementation on a video player.  %\feng{Simulation is also a type of experiment. Can we change ``experiment'' to ``real implementation''?}
Simulation allows us to evaluate a large set of parameters in a scalable manner. Real implementation provides insights under various system constraints.
In both cases, the network conditions are driven by
a set of traces captured from commercial LTE networks that allow reproducible runs as well as apple-to-apple comparison of different schemes.
We first describe the evaluation setup, and then compare PIA against several state-of-the-art schemes using simulation.
%rate-based approaches (RBH), buffer-based approach (BBA), and model-predicative-control based approach (MPC) and $pure$-PID using simulation experiments.
%We then evaluate the sensitivity of PIA to various parameters.
Last, we present real implementation results on a DASH player.

\subsection{Evaluation setup}


%\subsubsection{Network bandwidth traces}
\noindent{\textbf{Network bandwidth traces.}} We focus on LTE networks that dominate today's cellular access technology. For evaluation under realistic LTE network environments, we collected 50 network bandwidth traces from two large commercial LTE networks in the US. These traces were collected under a wide range of settings, including different times of day, different locations (in three U.S. states),
 %CT, NJ and NY) \feng{remove the state names due to anonymous requirement},
 and different movement speed (stationary, walking, local driving, and highway driving).
Each trace contains 30 minutes of one-second measurement of network bandwidth.
The bandwidth was measured as the throughput of a large file downloading from a well provisioned server on a mobile device.
%\feng{Describe how the bandwidth was measured.}
%The mean value of the traces varies from 1.1 to 20 Mbps, and the standard deviation varies from 0.9 to 17 Mbps.
Fig.~\ref{fig:trace-charact}(a) is a boxplot that shows the minimum, first quartile, median, third quartile, and maximum bandwidth of each trace, where the traces are sorted by the median bandwidth.
We see that the network bandwidth is indeed highly dynamic. For some traces, the maximum bandwidth is tens of Mbps while the minimum bandwidth is less than 10 Kbps.
%Fig.~\ref{fig:trace-charact}(b) shows the boxplot of the bandwidth prediction. Prediction The prediction is done every two seconds, as the harmonic mean of the past 20 s of bandwidth~\cite{}. We see

%\begin{figure}[h]
%    \centering
%        \includegraphics[height=2.5in]{figs/trace_characteristics_5_95.pdf}
%        \caption{Characteristics of Throughput}
%\label{fig:trace-charact}
%\end{figure}

%\tydubfigsingle{PIA/figs/trace_characteristics_box}{}{PIA/figs/trace_characteristics_predicterror_box}{}{Characteristics of the network bandwidth traces.}{trace-charact}
% \feng{subplot (a) the traces are sorted by throughput? If so say that.}}{trace-charact}
\begin{figure}[ht]
	\centering
	\subfigure[Heatmap.\label{subfig-1:heatmap}]{%
		\includegraphics[width=0.44\textwidth]{PIA/figs/trace_characteristics_box.pdf}
	}
	\subfigure[Histogram of ``heat" values.\label{subfig-2:heatmap_dist}]{%
		\includegraphics[width=0.44\textwidth]{PIA/figs/trace_characteristics_predicterror_box.pdf}
	}
	\caption{Characteristics of the network bandwidth traces.}
	\label{fig:trace-charact}
\end{figure}

%\subsubsection{Videos}
\smallskip
\noindent{\textbf{Video parameters.}}
We use three video bitrate sets: $\mathcal R_1=[0.35, 0.6, 1, 2, 3]$ Mbps, $\mathcal R_2=[0.35, 0.6, 1, 2, 3, 5]$ Mbps and $\mathcal R_3=[0.2, 0.4, 0.6, 1.2, 3.5, 5, 6.5, 8.5]$ Mbps. The first set is based on the reference for YouTube video bitrate levels (corresponding to 240p, 360p, 480p, 720p and 1080p respectively)~\cite{youtube-bitrate-levels}. The second set adds a higher bitrate level of 5 Mbps to the first set. The third set is based on Apple's HTTP Live Streaming standard~\cite{apple-bitrate-levels}. For each bitrate set, we further consider three variants with chunk size of 2, 4, and 8 s.
%, and video length as 5, 10 or 20 minutes, respectively.

\smallskip
\noindent{\textbf{ABR Schemes.}}
%\subsubsection{Adaptation Algorithms}
%We compare PIA with the three schemes.\\
We compare PIA against three other schemes.\\
%several widely adopted rate-based and buffer-based schemes. For all the schemes except for BBA, the network bandwidth at one point of time is estimated as the harmonic mean of the network bandwidth of the past $20$s. For all the schemes, the start-up latency $\delta$ is set to $5$, $10$ or $15$ s.
%PIA uses a look-ahead horizon of 5 chunks (i.e., $L=5$ in (\ref{eq:lms})).
%\begin{itemize}
  \BULLET {RB}: The bitrate is picked as the maximum possible bitrate that is below the predicted network bandwidth. This is a simple open-loop controller (see Section~\ref{sec:background}) serving as baseline.
%   (bandwidth prediction as a harmonic mean, as described later.

  \BULLET {BBA~\cite{huang2014buffer}}: This is a state-of-the-art buffer based scheme. We use BBA-0 (BBA-1 deals with variable bitrate (VBR) while for simplicity, we use constant bitrate (CBR) in simulation). The lower and upper buffer thresholds are $\theta_\text{low}=10$ s and $\theta_\text{high}=60$ s, respectively. The upper threshold is chosen to accommodate chunk size of 8s (for chunk size of 2 and 4 s, setting it to $30$ s leads to similar results).
      The corresponding buffer size is at most $60$ MB (considering the highest bitrate of 8 Mbps), reasonable even on mobile devices.
      %For the bitrate levels we consider, 60 s of buffer level leads to a buffer size of at most $60$ MB, which is reasonable even on mobile devices.
      We have empirically verified the above buffering setting works well on our dataset.
      %The buffer settings of BBA and PIA are comparable (see below), and we empirically verify they work well on our dataset.
      %\feng{Which BBA version do you use? Justify why you choose  $\theta_\text{low}=10$ s and $\theta_\text{high}=60$}

  \BULLET {MPC~\cite{yin2015control}}: The video bitrate is chosen by solving a discrete optimization problem by looking ahead for a horizon of 5 chunks (as suggested by the paper).

%  \item PIA: We set the target buffer level $x_r=30$ s or 60 s when video chunk size is 2 or 4 s; set $x_r=60$ s when video chunk size is 60 s. The larger buffer When  (weto accommodate When solving the
  \BULLET PIA: We set the target buffer level $x_r=60$ s that is compatible with the setting of BBA. The look-ahead horizon is set to 5 chunks (i.e., $L=5$ in (\ref{eq:lms})).
%\end{itemize}

For all the schemes, the start-up playback latency $\delta$ is set to $5$, $10$ or $15$ s.
%The above settings indeed provide apple-to-apple comparison
For BBA and MPC, their parameters are either selected based on the original papers, or configured by us based on the properties of the videos (e.g., chunk size and encoding rates) as justified above.

%\feng{Say two things: (1) this is indeed an apple-to-apple comparison because XXX, YYY, ZZZ are the same across all three schemes when we do the experiments. (2) We empirically (or how?) tune the parameters of BBA and MPC to ensure they work well on our dataset.}

\smallskip
\noindent{\textbf{Network bandwidth prediction.}}
%Among all the schemes that we evaluate, only BBA does not require network bandwidth prediction. For the rest of the schemes, the network bandwidth at one point of time is estimated as the harmonic mean of the network bandwidth of the past $20$s~\cite{jiang2012improving},
For the schemes that require network bandwidth estimation, it is set as the harmonic mean of the network bandwidth of the past $20$s. Harmonic mean has been shown to be robust to measurement outliers~\cite{jiang2012improving}. Fig.~\ref{fig:trace-charact}(b) shows the boxplot of the bandwidth prediction of the network traces.
Each box in the plot corresponds to the distribution of all prediction instances within a particular trace.
%\feng{It is unclear what each bar in the figure means. I assume it is the distribution of all prediction instances of a particular trace. Clarify this.}
The prediction is at the beginning of every second. As shown, the median prediction error is 20\% to 40\%, highlighting the challenges of accurate bandwidth prediction in LTE networks. %\feng{Sometimes we say ``network trace'', sometimes we say ``network profile''. Be consistent.}
% is a challenging problem, which is beyond the scope of our study.



\input{PIA/Kp-Ki}

\input{PIA/perf-comparison}

\input{PIA/sensitivity-new}

\vspace{-.05in}

\subsection{Computational overhead}
As described earlier, the computational overhead of PIA is much lower than that of MPC: for $m$ bitrate levels and horizon $L$, the complexity of MPC is $O(m^L)$, while the complexity of PIA is $O(mL)$.
%
On a commodity laptop with Intel i5 2.6GHz CPU and 16GB RAM, for 600 chunks (2-second chunk with bitrate set $\mathcal R_2$), the CPU time for MPC is 36.04 s, while the CPU time for PIA is 0.17 s, comparable to that of BBA (0.08s).




%Video bitrate recommended by YouTube and Apple.

\input{PIA/dash-results}


==> PIA/sensitivity-new.tex <==


\begin{figure*}[ht]
 \centering
 \subfigure[\label{subfig:videoAnalysisBitrate}]{%
      \includegraphics[width=0.3\textwidth]{PIA/figs/videoAnalysisBitrate}
    }
    \subfigure[\label{subfig:videoAnalysisBitrateChange}]{%
      \includegraphics[width=0.3\textwidth]{PIA/figs/videoAnalysisBitrateChange}
    }
    \subfigure[\label{subfig:videoAnalysisRebuffer}]{%
      \includegraphics[width=0.3\textwidth]{PIA/figs/videoAnalysisRebuffer}
    }
    \caption{Impact of video bitrate levels on performance (chunk size 2 s, video length 20 minutes, startup latency 10 s.)}
    \vspace{-.2in}
    \label{fig:video-analysis}
\end{figure*}

%\mysubsection{Impact of video bitrate sets}
\smallskip
\noindent{\textbf{Impact of video bitrate sets.}} Recall that the video bitrate set $\mathcal R_2$ has one higher bitrate level of 5 Mbps compared to $\mathcal R_1$.
%
We further investigate two more video bitrate sets $\mathcal R_4=[0.2, 0.35, 0.6, 1, 2, 3]$ Mbps, which has one lower bitrate of 0.2 Mbps compared to $\mathcal R_1$; and $\mathcal R_5=[0.2, 0.35, 0.6, 1, 2, 3, 5]$ Mbps, which has one lower and one higher video bitrate levels (of 0.2 and 5 Mbps) compared to $\mathcal R_1$. Fig.~\ref{fig:video-analysis} shows the results (the results of RB are omitted for better clarity).
The X axis is the video bitrate set ID, and each subplot corresponds to a metric.
%\feng{Say that the X axis is the video bitrate set ID, and each plot corresponds to a metric.}
%
For each metric, we plot the average value over all the network traces with 95\% confidence interval. We observe consistent trend for all three schemes (BBA, MPC, and PIA).
%
Comparing the results under $\mathcal R_1$ and $\mathcal R_2$, we see adding one higher bitrate level leads to higher average video bitrate, more bitrate changes, and more rebuffering;
%
comparing the results under $\mathcal R_1$ and $\mathcal R_4$,  we see adding one lower bitrate level maintains the average video bitrate while reduces bitrate changes and rebuffering;
%
comparing $\mathcal R_1$ and $\mathcal R_5$, we see adding both one lower and higher bitrate levels increases the average video bitrate and bitrate changes, while reduces the rebuffering.
%
In general, adding more bitrate levels helps improve at least one of the three metrics. Across the settings,
%the performance of PIA is stable: the 95\% confidence intervals for all the settings is small (\textbf{need to verify after the figure is updated}); it
PIA has the lowest bitrate switches, the lowest rebuffering, and comparable average bitrate compared to BBA and MPC.



\smallskip

%\feng{I would suggest remove Figure~\ref{fig:chunksize-analysis} and shorten the following paragraph, because Figure~\ref{fig:chunksize-analysis} does not look exciting and shows some negative results. Just say two things in the text: (1) we tested different chunk sizes and PIA consistently outperforms MPC and BBA in balancing the tradeoffs incurred by the three metrics. (2) For handling large chunks, the scheme can be further improved by adding preemption into PIA or introducing more bitrate levels.}

\noindent{\textbf{Impact of video chunk size.}}
We vary the video chunk size by setting it to 2, 4, and 8 s.
We found that for all chunk sizes, PIA consistently outperforms MPC and BBA in balancing the tradeoffs incurred by the three metrics. For example, for chunk size of 8 s, PIA's average playback bitrate differs from BBA and MPC only by 0.1\% and 3.2\%, respectively, while PIA reduces the rebuffering duration by 67\% and 68\% compared to those of BBA and MPC, respectively.









==> QUAD/abstract.tex <==
%\begin{abstract}


%Mobile video streaming is extremely popular, accounting for the bulk of traffic on cellular networks.

Streaming videos over cellular networks is highly challenging.\fengc{Streaming videos over cellular networks is particularly challenging due to highly dynamic network conditions. Today's Adaptive Bitrate (ABR) video streaming strategies
%ABR  strategies, widely  used for  OTT video  streaming,
focus on maximizing the Quality of Experience (QoE) and much less on reducing the data usage.}
Since cellular data is a relatively scarce resource, many video and network providers offer  options for users to exercise control over the amount of data consumed by video streaming. %These approaches typically work by limiting the  highest quality video track that the  ABR logic can select for any chunk.
Our study shows that existing data saving practices for Adaptive Bitrate (ABR) videos are suboptimal:
%such track-based limits
they often lead to highly variable video quality and do not make the most effective use of the network bandwidth. We identify underlying causes for this and propose two novel approaches to achieve better tradeoffs between video quality and data usage.
The first approach is Chunk-Based Filtering (CBF), which can be retrofitted to any existing ABR scheme. The second approach is QUality-Aware Data-efficient  streaming~(QUAD), a holistic rate adaptation algorithm that is designed ground up.
%
	We implement and integrate our solutions into
	%production-level
	two video player platforms (\texttt{dash.js} and ExoPlayer), and conduct thorough evaluations over emulated/commercial cellular networks using real videos.
%
%Our evaluations demonstrate that compared to the state of the art, the two proposed schemes achieve consistent video quality that is much closer to the user-specified target quality, far more efficient data usage, and lower stalls.
Our evaluations demonstrate that compared to the state of the art, the two proposed schemes achieve consistent video quality that is much closer to the user-specified target,
lead to far more efficient data usage, and incur lower stalls.
%\yanyuan{We will try to better summarize the main findings in the abstract. }



%\end{abstract}



==> QUAD/bing-command.tex <==

\usepackage{epsfig}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.25\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.16\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\vspace{-.1in}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsingledash}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.854\textwidth}
        \setlength{\epsfysize}{0.48\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.75\textwidth}
        \setlength{\epsfysize}{0.55\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\vspace{-.1in}
\end{figure}
}

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.87\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.10\textwidth}
%        \setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
        %\setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{1.10\textwidth}
        \setlength{\epsfysize}{0.78\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
\vspace{-0.1in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> carrier-aggre.tex <==
\subsection{Carrier Aggregation} \label{subsec:carrier-aggre}
%briefly discuss the effect of having two base stations (primary and secondary) serving one UE, and how the correlation results differ in this case.

In most of our measurements, a UE is served by a single base station at a given point of time. In some cases, we observe carrier aggregation (CA)~\cite{3gpp-ca}, where a UE is served by both two base stations (i.e., primary and secondary base stations) simultaneously. CA is defined in LTE Advanced (3GPP Release 10) in order to increase the bandwidth, and thereby increase the bitrate~\cite{3gpp-ca,Nokia-white-paper}. It has been launched in major LTE networks as of December 2014 and the coverage of CA in the major LTE networks continues to be expanded~\cite{att-ca,verizon-ca}. We observe CA in a residential area, which is occasionally served with CA.

%In principle, CA allows LTE-advanced UE to get allocation of downlink (DL) and uplink (UL) resources on the aggregated resource consisting of two or more Component Carriers (CC), which can be of different bandwidths. A UE can have more than one serving cells concurrently, one for each CC when CA is used.

In the presence of CA, we obtain radio parameters  as the average of both the primary and secondary base stations. We observe that the correlation between TBS and link bandwidth is very high (similar as that under the case without CA).  In the traces where CA is present in some portion of the trace, we obtain a time series on the number of base stations that are being used in each second (i.e., the value is either 1 or 2, depending on whether CA is present or not), and find that this time series has strong correlation with the time series of link bandwidth.

Our prediction approach can be applied to the case with CA by adding information related to the secondary base station and the number of base stations. We have verified that using TBS alone still provides accurate link bandwidth prediction in the presence of CA. Due to limited amount of trace, we leave further investigation to future work.

%In most cases, we observe a UE is served by a single base station. In some cases, we observe carrier aggregation~\cite{3gpp-ca} where a UE is served by both a primary and a secondary base station. Unless otherwise specified, the results are for a single base station. We briefly report the results under carrier aggregation in Section~\ref{subsec:carrier-aggre}.



==> dash.tex <==
\section{Video Streaming using LinkForecast} \label{sec:dash}
In this section, we present another case study that uses the link bandwidth prediction from LinkForecast for video streaming. We choose to use DASH (Dynamic Adaptive Streaming over HTTP)~\cite{stockhammer2011dynamic}, an adaptive streaming standard, because it is widely used and is compatible with video streaming delivered from conventional HTTP web servers. Specifically, we develop a LinkForecast based DASH scheme, referred to as \emph{L-DASH}, that dynamically adapts to link bandwidth changes. We next describe the design of L-DASH, and then evaluate its performance.


\subsection{L-DASH Design}
%Specifically, we develop a LinkForecast based DASH (Dynamic Adaptive Streaming over HTTP)~\cite{stockhammer2011dynamic} scheme, referred to as \emph{L-DASH}, that dynamically adapts to link bandwidth changes.
%DASH is an adaptive streaming standard that enables streaming of media content over the Internet delivered from conventional HTTP web servers.
In DASH, video content is broken into a sequence of small HTTP-based file segments. Each segment contains a short interval of playback time of the content, and is made available at a variety of bitrate. When fetching a segment, a DASH client selects the segment with the suitable bitrate to adapt to dynamic available bandwidth.

%We design and implement a L-DASH client that
L-DASH selects the bitrate of a segment based on the link bandwidth prediction from LinkForecast. Specifically, it simply fetches the segment with the highest bitrate that is below the bandwidth prediction.
We compare L-DASH with the default setting of an existing DASH client developed in~\cite{stockhammer2011dynamic}, which we refer to as the reference DASH client. This reference client uses exponentially weighted moving average to estimate bandwidth and then selects the corresponding segment bitrate. Specifically, let $\hat{b}_{i+1}$ denote the estimated bandwidth that is used to decide the bitrate for the $(i+1)$th segment. Let $b_i$ denote the average downloading speed for the $i$th segment that is obtained from measurement. Then $\hat{b}_{i+1}$  is estimated as
\begin{equation*}
\label{eq_cwnd}
\hat{b}_{i+1} = 0.55\cdot \hat{b}_{i} + 0.45\cdot b_{i}\,.
\end{equation*}



\subsection{Performance Evaluation}
The performance of L-DASH and the reference DASH client is evaluated in a trace-driven testing environment as described in Section~\ref{sec:environment}. Specifically, we assume that a UE uses either L-DASH or the reference DASH client to fetch video segments from a server; the network condition between the UE and the server is controlled by the traces that are collected from a commercial LTE network.
Our primary goal of comparing these two simple schemes is to demonstrate the benefits of link bandwidth prediction from LinkForecast. A comprehensive evaluation of L-DASH and other variants of adaptation schemes is left as future work.

For the video content, we use the trailer of Sintel, a computer animated video available from the Xiph.Org Foundation~\cite{xiph}. The length of the video is one minute. We encode the video according to the H.264/MPEG-4 AVC compression format. The resolution is 1920x1080p and the frame rate is 24 frames per second. The video is divided into 30 segments, each of 2 seconds. Each segment is then encoded at 16 different bitrates, ranging from $1,000$ to $9,000$ kbps, with the increment of $500$ kbps. The rationale for choosing 2-second segments is that it allows flexibility for adapting to bandwidth fluctuations.
We set a maximum buffer size of 5 seconds at the client (i.e., the client stops buffering if it already has 5 seconds of video in the buffer), so the client may smoothen the video playback in the case of temporary link disruptions without buffering too much data.

%While many factors may impact the user experience with video streaming applications, we evaluate only the following most widely used \emph{objective} metrics: Peak Signal-to-Noise Ratio (PSNR), Video Quality Metric (VQM). And we also evaluate the number of interruptions (freezes) during video playback.

We use three performance metrics: two are objective metrics, Peak Signal-to-Noise Ratio (PSNR) and Video Quality Metric (VQM)~\cite{vqmpaper}, and the third is the number of interruptions (freezes) during video playback. PSNR is one of the most widely used metrics. It is derived by setting the mean squared error (MSE) in relation to the maximum possible value of the luminance. Compared with PSNR, VQM is shown to have a better correlation with subjective video quality assessment. The number of freezes can significantly affect user perceived experience during video playback, and hence we also use the number of freezes as a performance metric.

In our test environment, we create a 30-minute trace by concatenating two traces collected from a commercial LTE network, one trace of 18 minutes collected by driving on highway, and the other of 12 minutes collected in a static office environment. The one-minute video is played repeatedly for 30 times over the 30-minute long trace.

\dubfigsingledash{fig/dash_low2}{reference DASH client}{fig/dash_high2}{L-DASH}{Two screenshots that demonstrate the visual difference rendered by the reference DASH client and L-DASH (VQM for the reference DASH client is 0.51; VQM for L-DASH is 0.24).}{fig_demo2}

\subsubsection{PSNR}
Fig.~\ref{fig:PSNR} shows the PSNR of L-DASH and the reference DASH client for a sample video play of $1,200$ frames (50 seconds). We observe that L-DASH provides equal or better video quality than the reference DASH client most of the time.
While playing the video over the 30-minute long trace, L-DASH achieves up to 6.3 dB improvement in PSNR compared to the reference DASH client; the average improvement in PSNR is 1.5 dB (45.1 dB vs 43.6 dB).
The improvement is because L-DASH can quickly adjust to dynamic bandwidth: when the predicted bandwidth is high, it adjusts quickly by fetching a high bitrate segment; when the predicted bandwidth is low, it adjusts quickly by fetching a low bitrate segment. The reference DASH client, however, relies heavily on historic measurements, and does not adapt to the highly dynamic cellular conditions quickly.

\begin{figure}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/psnr}
\caption{The PSNR for L-DASH and the reference DASH client (higher is better).}
\label{fig:PSNR}
\end{center}
\end{figure}




\subsubsection{VQM}
Fig.~\ref{fig:vqm} plots an example result of VQM (lower is better) for L-DASH and the reference DASH client. In this example, L-DASH achieves similar or better VQM, and hence better perceptual quality. To demonstrate the results visually, Fig.~\ref{fig:fig_demo2} displays two screenshots, corresponding to the 54-th frame in Fig.~\ref{fig:vqm}, where the VQM for the reference DASH client is 0.51, while the VQM for L-DASH is 0.24. Over the 30-minute long trace, L-DASH achieves an average improvement of 15\% in VQM (0.44 vs 0.53).
%For all the traces we tested, L-DASH achieves an average improvement of 15\% (0.44 vs 0.53).

\begin{figure}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/vqm}
\caption{The VQM distortion for L-DASH and the reference DASH (lower is better).}
\label{fig:vqm}
\end{center}
\end{figure}


\subsubsection{Freezes}
While playing the one-minute long video 30 times over the 30-minute long trace, the average number of freezes is 0.9 per video play when using L-DASH, while the average number of freezes is 5.2 per video play when using the reference DASH client. Most of the freezes are caused by overestimating link bandwidth. For L-DASH, significant overestimation is rare as presented in Section~\ref{sec:pred_performance}. For the reference DASH client, however, overestimation happens more frequently as it heavily relies on historic measurements, which become obsolete quickly in rapidly varying cellular link conditions.


\iffalse
\subsection{Performance Evaluation}

For the video content, we used the Sintel trailer animated video from the Xiph.Org Foundation~\cite{xiph}. The length of the video is one minute. We encode the video into the H.264/MPEG-4 AVC compression format. The resolution is 1920x1080p and the frame rate is 24 frames per second. The video is divided into 30 segments, each of 2 seconds. Each segment is then encoded at bitrates ranging from 1000 to 9000 kbps. The reason we choose 2-second segments is because it allows flexibility for adapting to bandwidth fluctuations.
We set a maximum buffer size of 5 seconds (i.e., the client stops buffering if it already has 5 seconds of video in the buffer), so the client may smooth over temporary link disruptions without buffering too much data.

Although there are many factors that may have impacts on the user experience with video streaming applications. In this section, we evaluate only the following most widely used \emph{objective} metrics: Peak Signal-to-Noise Ratio (PSNR), Video Quality Metric (VQM). And we also evaluate the number of interruptions (freezes) during video playback.

%We use a widely adopted standard video quality measurement tool~\cite{vatolin2009msu} to assess the objective video quality of LinkForecast and original DASH.
%In order to compare the performance of L-DASH client and the reference DASH client, for each experiment we replay the exact trace for both clients and record the entire video that is played. We repeat the experiments 100 times using different cellular traces.

%To best compare the video quality among different schemes, we take the following steps. (1) We replay the same cellular trace for L-DASH and the reference DASH, so that the videos are played in the exactly same network condition. (2) After the video playback is finished, we reconstruct the video with the segments that have been fetched according to the log file. (3) We compare the video quality of the reconstructed videos with the original uncompressed version. (4) We repeat the experiment for different traces and collect the overall results.

\subsubsection{PSNR}

The peak signal-to-noise ratio (PSNR) is one of the most widely used metric. PSNR is derived by setting the mean squared error (MSE) in relation to the maximum possible value of the luminance.

Fig.~\ref{fig:PSNR} shows the PSNR comparison for L-DASH and the reference DASH client for a . It can be observed L-DASH provides equal or better video quality than the reference DASH client for most of the time.
For all the traces we tested, L-DASH achieves an average improvement in PSNR of 1.5 dB (45.1 dB vs 43.6 dB), with a maximum improvement of 6 dB. The improvement is because L-DASH can quickly fetch a higher bitrate segment when it predicts the link bandwidth is high. The reference DASH client, however, relies heavily on the historic measure, and it thus does not adapt to the highly dynamic cellular conditions.

\begin{figure}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/psnr}
\caption{The PSNR for LinkForecast and the original DASH scheme.}
\label{fig:PSNR}
\end{center}
\end{figure}


\subsubsection{VQM}

Another video quality metric, VQM~\cite{vqmpaper}, is shown to have a better correlation with subjective video quality assessment. Fig.~\ref{fig:vqm} plots an example results of VQM (lower is better) for L-DASH and the original DASH. In this example, L-DASH achieves similar or better VQM. i.e., a better perceptual quality. To demonstrate the visual effect of VQM, we show the screenshots in Fig.~\ref{fig:fig_demo2} where the VQM differences is high.

\dubfigsingledash{fig/dash_low2}{reference DASH client}{fig/dash_high2}{L-DASH}{VQM demo. On the left is when VQM is 0.24 with reference DASH client, and on the right is when VQM is 0.51 with L-DASH}{fig_demo2}
\begin{figure}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/vqm}
\caption{The VQM distortion for L-DASH and the reference DASH (lower is better).}
\label{fig:vqm}
\end{center}
\end{figure}



%\dubfigsingledash{fig/dash_low}{reference DASH client}{fig/dash_high}{L-DASH}{reference DASH}{fig_demo1}

For all the traces we tested, L-DASH achieves an average improvement of 15\% (0.44 vs 0.53).

\iffalse
\begin{figure}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/dash_low}
\newline{\small (a) Reference DASH client}
\includegraphics[width=3.2in]{fig/dash_high}
\newline{\small (a) LinkForecast}
\caption{The PSNR for LinkForecast and the original DASH scheme.}
\label{fig:PSNR}
\end{center}
\end{figure}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=3.2in]{fig/dash_low2}
\newline{\small (a) Reference DASH client}
\includegraphics[width=3.2in]{fig/dash_high2}
\newline{\small (a) LinkForecast}
\caption{The PSNR for LinkForecast and the original DASH scheme.}
\label{fig:PSNR}
\end{center}
\end{figure*}

\fi




\subsubsection{Freezes}

Another key metric that affects the user experience is the frequency and duration of freezes in video playback. We count the number of video freezes by reading the the log of both DASH clients.
%The number of video freezes increases as the playback continues.
For all the cellular traces we tested, one interruption per minute of video play back was observed with L-DASH, while with the reference DASH client, we experience 5 interruptions per minute. Most of the freezes are caused by overestimating link bandwidth. For L-DASH, overestimation is rare as presents in Section~\ref{sec:pred_performance}. For the reference DASH client, however, overestimations are more frequent as it heavily relies on the historic measurement which is obsolete quickly in rapidly varying cellular link conditions.
\fi

%uring the 375-second playback period with LinkForecast; while for the reference DASH client, for the same playback period, an average of 4 interruptions were observed.

%\subsection{Summary}
%In this section, we presented a modified DASH client that






==> data.tex <==
\section{Data Collection Methodology}
\label{sec_data_collection}


We collect data from two largest commercial LTE networks in the US. Specifically, we collect two types of information, cellular link bandwidth and lower layer information, simultaneously. These two types of information will be used for the following two purposes : (i) they will be used to study the correlation between link bandwidth and various radio information to identify key parameters that can be used for link bandwidth prediction in Section~\ref{sec:correlation}; and (ii) the radio information will be used to predict link bandwidth and be compared with the collected link bandwidth (treated as the ground truth) to evaluate the accuracy of the prediction framework in Section~\ref{sec:prediction}.

We next describe how we obtain these two types of information.
Link bandwidth represents the bandwidth that is available to a UE over the cellular link. It is not directly perceivable, and has to be obtained through active measurement.
We use a purposely written program to send a certain amount of data that can saturate the link while not causing very long queuing delays. While the link is saturated, we use a packet sniffer to record the network traffic.

Lower layer information is available at a UE. However, currently commodity UEs do not expose the information to the operating system at a fine granularity (see more discussion in Section~\ref{sec:discuss}). We use QxDM (Qualcomm eXtensible Diagnostic Monitor), a tool developed by Qualcomm~\cite{QXDM}, to record various radio information in real time for phones with Qualcomm chipsets. Specifically, to record QxDM traces, we connect a phone using a USB cable to a laptop that runs QxDM. QxDM communicates with the phone through a diagnostic port and records the traces, where the various radio information is logged periodically, with the intervals varying from tens of milliseconds to hundreds of milliseconds.

Furthermore, in order to make sure that the extra data collection overhead does not affect the normal operation of the phone. We measured the CPU usage on a phone when collecting radio information with QxDM, and find that QxDM does not cause any noticeable increase in CPU usage. In other words, collecting radio information in real-time does not affect the performance of the phone.

\iffalse
The first piece of information we are interested in is the available link bandwidth. Obtaining the cellular link bandwidth is challenging, as it is not directly perceivable. Therefore, we approximate the link bandwidth by saturating the link with a purposely written client-server program (as used in~\cite{Winstein:2013:SFA:2482626.2482670}). The client runs on a phone and on the server has a good, low-delay (< 20 ms) Internet connection to the cellular carrier.

During the measurement, the sender keeps a window of $N$ packets in flight to the receiver, and adjusts $N$ in order to keep the observed RTT greater than 750 ms (but less than 3000 ms). The theory of operation is that if packets are seeing more than 750 ms of queueing delay, the link is not starving for offered load.
In the meantime we use a packet sniffer to record the traffic traces on the smartphones. From the traces, we can obtain the maximum bandwidth at any point of time and we use that as an approximation of link bandwidth. As a sanity check, we also use iPerf to measure the bandwidth in UDP mode. The results are consistent with the tool we used.
All the network traces collected can be replayed to create a reproducible cellular network environment for performance evaluation for evaluation purposes (see Section~\ref{simu}).

Secondly, we also need to keep track of various radio related information such as signal strength, modulation scheme, etc. To collect the information, we connect the phones to a laptop and use the tool named QxDM from Qualcomm~\cite{QXDM} to record various radio parameters in real time. QxDM communicates with the phones through diagnostic port and generates the radio traces.
\fi

\section{Data Set}
\label{sec:dataset}

We have performed extensive measurements during a period of 15 months (from July 2014 to October 2015) in two major US commercial LTE networks, AT\&T and Verizon. The data are collected using seven different phones, Samsung S3, S4, S5, Note 3 and HTC M8 in AT\&T network, and Samsung S4 and S5 in Verizon networks, at locations in three states CT, NY and NJ in the US.
%The smartphones we used are produced by major manufacturers between 2012 to 2015.

We collected around 50 hours of data, and 200 GB of traffic traces under a wide range of scenarios, including different times of a day, different locations (residential, campus, office, etc.), and different movement speed (stationary, walking, local driving, and highway driving). Tables~\ref{table_data1} and \ref{table_data2} list the majority of the data collected in AT\&T and Verizon networks, respectively. For clarity, only the data collected by Samsung Note 3 in AT\&T network is marked with time.
%The rest of the data
%Tables~\ref{table_data1} and \ref{table_data2} highlights the major data to be evaluated in Section~\ref{sec:correlation} and Section~\ref{sec:prediction}, which contains four devices running on two commercial LTE networks.
%We also used the data collected from other devices in various scenario (table omitted) mainly for data sensitivity test to be described in Section~\ref{sec:sensitivity}.
%In total, from the eight devices we have collected around 50 hours of data, and 200 GB of traffic traces.
Because the traces were collected at different times and places, the measurements cannot be used to compare different commercial services head-to-head.

%Each scenario contains multiple traces that are collected at different times of a day and over different days. The highway driving scenario includes traces going from the campus to two cities, 140 and 30 miles away, respectively.
%The numbers of unique eNodeBs in campus, residence, local driving and highway driving scenarios are 3, 3, 14 and 57 respectively. The total number of unique eNodeBs over all the scenarios is 67. %The number of eNodeBs included in the traces is over 67.

%Our data set has the limitation that it is collected from a single LTE network, and the two phones' chipsets are from the the same vender (Qualcomm). On the other hand, the network is one of the largest in the United States, and Qualcomm is the dominant LTE chipset provider. In addition, the approach we use is based on the fundamental mechanisms of LTE networks, and is expected to be applicable to other networks.
%We are only able to use QxDM on Andriod phones (not on iPhones or other phones).  (it produces ?? of Android phones).
%Investigation using more cellular networks and phones from other manufactures is left as future work.

%Table~\ref{table_data1} summarizes the data collected using Phone 1. It contains a total of 10.8 hour of data, over 40 GB of traffic traces and over 5 GB of QxDM radio traces. Each scenario contains multiple traces that are collected at different times of a day and/or over different days. Table~\ref{table_data2} summarizes the data collected using Phone 2. It contains less amount of data. Our main purpose is to understand the difference between these two phones. Therefore, the data for Phone 2 contain multiple traces, each collected right after a trace is being collected using Phone 1. The total duration is 3.2 hours, with around 8.8 GB of traffic traces and 1.3 GB of QxDM radio traces.


%remove some info, merge two highway driving traces

%wb, 12/16/2015
\begin{table}[]
	\centering
	\caption {Data collected from AT\&T network.}
	\label{table_data1}
	\begin{tabular}{|l|l|r|r|}
		\hline
		Phone                           & Scenario          & Duration & Traffic                      \\ \hline
		\multirow{6}{*}{Samsung Note 3} & Static (day)      & 3.3 hr   & 9.8 GB                       \\ \cline{2-4}
										& Static (night)    & 2.5 hr   & 7.8 GB                       \\ \cline{2-4}
										& Walking (day)     & 1.5 hr   & 4.3 GB                       \\ \cline{2-4}
										& Walking (night)   & 0.7 hr   & 2.2 GB                       \\ \cline{2-4}
										& Local driving     & 1.2 hr   & 4.7 GB                       \\ \cline{2-4}
										& Highway driving   & 1.4 hr   & 9.8 GB                       \\ \hline
		\multirow{3}{*}{HTC M8}         & Static (day)      & 6.6 hr   & 16.5 GB                      \\ \cline{2-4}
										& Static (night)    & 2.7 hr   & \multicolumn{1}{l|}{15.5 GB} \\ \cline{2-4}
										& Local driving     & 0.6 hr   & 2.1 GB                       \\ \hline
		Samsung S3, S4, S5              & various scenarios & 4.5 hr   & 21.2 GB                      \\ \hline
	\end{tabular}
\end{table}

\iffalse
\begin{table}[t]
\centering
    \caption {Data collected from AT\&T network.}
\begin{tabular}{|l|r|r|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & Traffic   \\\hline \hline
  Static (Samsung Note 3) & 5.7 hr  & 17.6 GB  \\ \hline
  Walking (Samsung Note 3) & 1.9 hr & 4.3 GB \\ \hline
%  walking (residence) & 0.5hr & 1GB () \\ \hline
  Local driving (Samsung Note 3)  & 1.2 hr & 4.7 GB \\ \hline
  Highway driving (Samsung Note 3)  & 1.4 hr & 9.8 GB  \\ \hline \hline
  Static (HTC M8) & 9.3 hr  & 32.0 GB \\ \hline
  Local driving (HTC M8)  & 0.6 hr & 2.1 GB \\
  \hline
\end{tabular}
    \label{table_data1}
\end{table}
\fi

\begin{table}[]
	\centering
	\caption {Data collected from Verizon network.}
	\label{table_data2}
	\begin{tabular}{|l|l|r|r|}
		\hline
		Phone                       & Scenario                     & Duration & Traffic \\ \hline
		\multirow{4}{*}{Samsung S4} & Static (day)                 & 5.7 hr   & 25.7 GB \\ \cline{2-4}
									& Static (night)               & 2.9 hr   & 14.7 GB \\ \cline{2-4}
									& Local driving                & 1.5 hr   & 2.0 GB  \\ \cline{2-4}
									& Highway driving              & 0.8 hr   & 2.2 GB  \\ \hline
		\multirow{4}{*}{Samsung S5} & Static (day)                 & 6 hr     & 29 GB   \\ \cline{2-4}
									& Static (night)               & 3 hr     & 20 GB    \\ \cline{2-4}
									& Local driving (Samsung S5)   & 1.2 hr   & 3.1 GB  \\ \cline{2-4}
									& Highway driving (Samsung S5) & 0.9 hr   & 4.5 GB  \\ \hline
	\end{tabular}
\end{table}

\iffalse
%4 million samples
We have performed extensive measurements during a period of more than one year (from July 2014 to October 2015). The data are collected using multiple Android smartphones from several major smartphone manufacturers, and over two of the largest commercial cellular networks (AT\&T and Verizon) in the US. Table~\ref{table:phones} lists the detailed specifications of the devices we used.

\iffalse
\begin{table}[t]
\centering
    \caption {Devices Specification}
\begin{tabular}{|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Model                 & Chipset                               & Carrier           & Release Date   \\\hline \hline
  Samsung Galaxy S3     & Qualcomm Snapdragon S4                & AT\&T             & May 2012 \\ \hline
  Samsung Galaxy S4     & Qualcomm Snapdragon 600               & AT\&T \& Verizon   & March 2013  \\ \hline
  Samsung Galaxy S5     & Qualcomm Snapdragon 801 MSM8974-AC    & Verizon           & April 2014 \\ \hline
  Samsung Galaxy Note 3 & Qualcomm Snapdragon 800 MSM8974       & AT\&T             & September 2013 \\ \hline
  LG G3                 & Qualcomm Snapdragon 801 MSM8974-AC    & Verizon           & May 2014 \\ \hline
  HTC One (M8)          & Qualcomm Snapdragon 801 MSM8974-AB    & AT\&T             & March 2014\\ \hline
\end{tabular}
    \label{table:phones}
\end{table}
\fi

\begin{table}[t]
\centering
    \caption {Devices Specification}
\begin{tabular}{|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Model                 & Chipset                   & Carrier           & Release Date   \\\hline \hline
  Samsung Galaxy S3     & Qualcomm  S4    & AT\&T             & May 2012 \\ \hline
  Samsung Galaxy S4     & Qualcomm  600   & AT\&T \& Verizon  & Mar. 2013  \\ \hline
  Samsung Galaxy S5     & Qualcomm  801   & Verizon           & Apr. 2014 \\ \hline
  Samsung Galaxy Note 3 & Qualcomm  800   & AT\&T             & Sep. 2013 \\ \hline
  Samsung Galaxy S6 Edge+& Samsung Exynos  & Verizon           & Aug. 2015 \\ \hline
  LG G3                 & Qualcomm  801   & Verizon           & May 2014 \\ \hline
  HTC One (M8)          & Qualcomm  801   & AT\&T             & Mar. 2014\\ \hline
\end{tabular}
    \label{table:phones}
\end{table}

%One is Samsung Galaxy Note 3, the other is Samsung Galaxy S3, referred to as Phone 1 and Phone 2, respectively. Both phones are equipped with Qualcomm chipsets. Phone 1 is more recent and powerful than Phone 2 (they use Qualcomm Snapdragon 800 and MSM8960 processors, respectively). For our purpose, it is not necessary to use a wide variety of phones since we found that most phones with Qualcomm chipsets provide similar set of radio information, which we collect using a Qualcomm analysis tool as described earlier. Both phones use LTE for data service in the large commercial LTE network that we chose to collect measurements.

Furthermore, since link bandwidth may vary depending on time, location, and mobility, we collect in from a wide range of settings, including different times of a day, at different locations (e.g., university campuses, residential area), and different movement speed (stationary, walking, local driving, and highway driving). Table~\ref{table_data1} summarizes the data collected using Phone 1. It contains a total of 10.8 hour of data, over 40 GB of traffic traces and over 5 GB of QxDM radio traces. Each scenario contains multiple traces that are collected at different times of a day and/or over different days. Table~\ref{table_data2} summarizes the data collected using Phone 2. It contains less amount of data. Our main purpose is to understand the difference between these two phones. Therefore, the data for Phone 2 contain multiple traces, each collected right after a trace is being collected using Phone 1. The total duration is 3.2 hours, with around 8.8 GB of traffic traces and 1.3 GB of QxDM radio traces.

\iffalse
%a table listing the data
\begin{tabular}{|l|l|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & \# of traces & Trace size  & cells & carrier aggregation \\
  static (office) & 1.7hr & 3 & 5.4GB () & 1-2 & N \\
  static (residence) & 2.5hr & 9 & 5GB () & 3 & Y \\
  walking (campus) & 1hr & 3 & 2GB () &  & N \\
  walking (residence) & 0.5hr & 1 & 1GB () &  & Y \\
  driving (local) & 1hr & 6 & 5GB () & 11 & N \\
  driving (highway 1) & 1hr & 2 & 7.5GB () & 22 & N \\
  driving (highway 2) & 1.2hr & 2 & 2GB () &  & N \\
  \hline
\end{tabular}
\fi

%remove some info, merge two highway driving traces
\begin{table}[t]
\centering
    \caption {Data collected using Phone 1.}
\begin{tabular}{|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & Traffic & QxDM  \\\hline \hline
  static (campus, day) & 1.7 hr  & 5.0 GB & 0.6 GB\\ \hline
  static (campus, night) & 1.5 hr  & 4.8 GB & 0.6 GB \\ \hline
  static (residence) & 2.5 hr & 7.8 GB & 1.0 GB \\ \hline
  walking (campus, day) & 1.5 hr & 4.3 GB & 0.6 GB \\ \hline
  walking (campus, night) & 1.0 hr & 2.7 GB & 0.4 GB \\ \hline
%  walking (residence) & 0.5hr & 1GB () \\ \hline
  local driving  & 1.2 hr & 4.7 GB & 0.6 GB\\ \hline
  highway driving  & 1.4 hr & 9.8 GB & 1.2 GB \\
  \hline
\end{tabular}
    \label{table_data1}
\end{table}

\iffalse
\begin{table}[t]
\centering
    \caption {Data collected using Phone 1.}
\begin{tabular}{|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & Trace size  \\\hline \hline
  static (campus, day) & 1.7 hr  & 5.0 GB (0.6 GB) \\ \hline
  static (campus, night) & 1.5 hr  & 4.8 GB (0.6 GB) \\ \hline
  static (residence) & 2.5 hr & 7.8 GB (1.0 GB) \\ \hline
  walking (campus, day) & 1.5 hr & 4.3 GB (0.6 GB) \\ \hline
  walking (campus, night) & 1.0 hr & 2.7 GB (0.4 GB) \\ \hline
%  walking (residence) & 0.5hr & 1GB () \\ \hline
  local driving  & 1.2 hr & 4.7 GB (0.6 GB) \\ \hline
  highway driving  & 1.4 hr & 9.8 GB (1.2 GB) \\
  \hline
\end{tabular}
    \label{table_data1}
\end{table}
\fi


\begin{table}[t]
\centering
    \caption {Data collected using Phone 2.}
\begin{tabular}{|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & Traffic & QxDM  \\\hline \hline
  static (campus, day) & 1.0 hr  & 2.7 GB & 0.4 GB \\ \hline
  static (campus, night) & 1.2 hr  & 3.5 GB & 0.5 GB \\ \hline
  walking (campus, day) & 1.0 hr  & 2.6 GB & 0.4 GB \\ \hline
  \hline
\end{tabular}
    \label{table_data2}
\end{table}


\iffalse
\begin{table}[t]
\centering
    \caption {Data collected using Phone 2.}
\begin{tabular}{|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Scenario & Duration & Trace size  \\\hline \hline
  static (campus, day) & 1.0 hr  & 2.7 GB (0.4 GB) \\ \hline
  static (campus, night) & 1.2 hr  & 3.5 GB (0.5 GB) \\ \hline
  walking (campus, day) & 1.0 hr  & 2.6 GB (0.4 GB) \\ \hline
  \hline
\end{tabular}
    \label{table_data2}
\end{table}
\fi

\fi


==> discuss.tex <==
\section{Discussion}
\label{sec:discuss}

In this section, we discuss a couple of practical issues, one related to using our approach when a UE is served simultaneously by multiple base stations (a practice that has started to be adopted by commercial carriers~\cite{att-ca,verizon-ca}), and the other related to the implication of our study in practice.
\input{carrier-aggre}

%\subsection{Network Level Information versus Radio Information}

\subsection{Deployment Issues}
We use QxDM to gather fine-granularity (at the interval of tens of or hundreds of milliseconds) radio information with the goal of exploring the performance space. Specifically, the goal is to identify what information is critical for accurate link bandwidth prediction and at what granularity the information is useful. A natural question is, since such information is not yet accessible on commodity phones (indeed we have to resort to QxDM), how to use our approach in practice.

%While not all radio information that we have identified is exposed to the operating systems, we observe that
We make the following two comments. First, a recent trend is that lower-layer information becomes increasingly accessible. Specifically, current mobile processors and chipsets (e.g., Qualcomm Snapdragon processors) provide ways to read various parameters from the radio interface of a mobile device in real time; mobile operating systems are exposing more radio related APIs (e.g., Android has included APIs that provide multiple signal strength related information);
and manufacturers are providing lower level information to users (e.g., the service menu on Samsung smartphones). We hope that our results can serve to accelerate the trend in making radio information
%critical radio layer information that is helpful for link bandwidth prediction
accessible at mobile devices. Secondly, our results indicate that even a small set of information at coarse granularity is useful for obtaining accurate link bandwidth prediction. Even if not all radio information is made available at fine granularity in the near future, we hope our results can incentivize the practitioners to make a small set of critical radio information accessible at coarse granularity.

%To obtain an estimate on the overhead of

%We find that even a small set of information at coarse granularity is useful for obtain accurate prediction. While some of the radio information we identified is not yet accessible on commodity smartphones, we hope that our results can serve to accelerate the trend in making more radio layer information accessible at mobile devices.

Last, it is worth mentioning that the prediction performance of LinkForecast cannot be directly used as an indicator for transport or application layer performance. For instance, if a low bandwidth link is mis-predicted as having high bandwidth, it is very likely to cause a transport protocol or an application to send more data than the link can handle, and thus creates a large queue, which may take seconds to be drained. We will investigate using LinkForecast in designing transport protocols in Chapter~\ref{chapter:ltp}.


==> intro.tex <==


%\section{Background and Motivation}
\iffalse
\chapter{Introduction}
\label{chapter:intro}
 Cellular infrastructures have been evolving at a fast speed. From a recent report on global network traffic~\cite{index520862global}, it is projected that the overall mobile data traffic is expected to grow to 24.3 exabytes per month by 2019, with a compound annual growth rate (CAGR) of 57\%.

\begin{figure}[h]
\begin{center}
\includegraphics[width=5in]{fig/cisco}
\caption{Cisco Forecasts 24.3 Exabytes per Month of Mobile Data Traffic by 2019.}
\label{fig:arch}
\end{center}
\end{figure}

The current 4G LTE (Long Term Evolution) cellular networks provide significantly higher data rate and lower network latency than earlier generation systems. The advances provided by LTE, however, may not be fully utilized by upper-level protocols and applications due to the rapidly varying cellular link conditions. For instance, a recent large-scale study of LTE networks
~\cite{huang2014buffer}
shows that, for 71.3\% of the large flows, the bandwidth utilization rate is below 50\%. Supporting delay-sensitive applications such as VoIP, video streaming and interactive applications in LTE networks remains to be a difficult task. With the wide deployment of LTE networks, it becomes increasingly important to understand cellular link characteristics, identify performance issues, and improve the performance of upper-level protocols and applications in LTE networks.

\section{LTE }
\label{sec:lte_basics}


\subsection{Characteristics of LTE networks}

One distinguishing characteristics of cellular networks is their rapidly changing channel conditions, which may cause the link bandwidths to vary in orders of magnitude within seconds.
%For instance, in the TCP slow start phase, congestion window increases only after each received ACK. They work well on relatively stable links, but they do not react to the fast changing cellular link quickly.
This creates two problems: low link utilization, and long delays.
%. On one hand, it results in low utilizations of cellular links.
%On the other hand, it creates longer delays.
If too much data is sent due to an improper reaction to a reduced link capacity, a queue will be built up quickly. For instance, as shown in Fig.~\ref{intro}, the two widely adopted TCP variants, Cubic (the default in Linux) and Vegas, do not perform well in LTE networks. We can observe from the figure that the link capacity (the grey area) is not effectively utilized (see Section~\ref{sec_data_collection} for details on link capacity estimation). In this example, the average utilization achieved by the two TCP variants are 74\% and 45\%, respectively.

Another feature of LTE networks is that the base station, i.e., eNodeB, in the LTE networks maintains independent buffers for different clients.
In downlink direction, the eNodeB maintains buffers per UE containing dedicated data traffic. Similarly, in the uplink each UE has data queues corresponding to uplink logical channels.
In this condition, users are rarely subject to standing queues accumulated by other users.
%In other words, the queuing delay is largely self-inflicted. This unique characteristic gives us an opportunity to optimize network performance on client side directly.
Therefore, the latency that a UE observes primarily depends on its own packet transmissions, independent of the actions of other users.
%In a network where two independent users share access to a queue feeding into a bottleneck link, one user can inflict delays on another. No end-to-end protocol can provide low-delay service when a network queue is already full of somebody else’s packets. But when queueing delays are largely self-inflicted, an end-to-end approach may be possible.



\section{New Protocol and Application Design}

The accurate link bandwidth prediction can in turn be utilized by upper-level protocols and applications to improve their performance.
We explore new designs for transport protocols in LTE networks that directly utilize the real time link bandwidth prediction.
Evaluation using real-world traces demonstrates that our protocol outperforms traditional TCP protocols, achieving both high throughput and low delay at the same time. Compared with a recent transport protocol that is designed for cellular networks, our protocol achieves similar or better performance while our protocol is much simpler and does not require long training period. Our study highlights the benefits of using radio layer information when designing higher layer protocols for cellular networks.

Meanwhile, real-time entertainment (comprised of streaming video and audio) continues to be the largest traffic category on virtually every network.
For instance, during the evening peak hours (8pm - 1am EDT), well over 50\% of US Internet traffic is video streamed from Netflix and YouTube~\cite{sandvine}.
Among the video streaming traffic, an increasing fraction is driven by video consumption on mobile phones and tablet devices on mobile networks, thanks to a significantly higher link bandwidth enabled by the 4G LTE networks.

Many recent studies have highlighted that the user-perceived Quality of Experience (QoE) plays a critical role for Internet video streaming application. The key metrics involves average video quality, duration of rebuffering, number of video quality switches, etc. However, due to the rapidly varying link condition in cellular network, it remains to be a big challenge to provide users with a seamless multimedia experience with high QoE.
Specifically, achieving good QoE in adaptive video streaming requires maximizing the average video bitrate, minimizing the amount of rebuffering and bitrate variation. These three optimization goals are at odds with each other, and are extremely difficult to balance in cellular networks with highly dynamic bandwidth.

Many recent studies have provided solutions for tackling this problem (e.g.~\cite{huang2012confused, tian2012towards,jiang2012improving,jiang2012improving, de2013elastic, huang2014buffer, yin2015control}). Some studies try to find better ways to estimate the future throughput~\cite{jiang2012improving}, some try to augment the throughput prediction with buffer information~\cite{de2013elastic, tian2012towards} and some other~\cite{huang2014buffer} even argue against capacity estimation and propose to use buffer occupancy solely. (A more detailed overview of related work can be found in Section~\ref{sec:abr_related}).

While previously studies have shown key limitations of state-of-art solutions and proposed a wide range of heuristic solutions, most of the solutions are heuristic and there is still a lack of understanding about their inherent mechanisms and how to properly tune their system parameters. In order to further understand the adaptive video streaming in cellular network, we begin by formulating the existing approaches in a control-theoretic framework. Then we analyze their system characteristics and identify their limitations. After that, we design a PID based feedback control framework and investigate the system behavior by conducting comprehensive evaluations under numerous controller settings and various real-world cellular traces. By examining the evaluations results, we provide a guideline for tuning the adaptive video streaming system. Following the guideline our system shows that the system behavior is consistent with the design and it outperforms state-of-art video streaming solutions. We hope our work can shed some light on the video adaptation design for the cellular networks.

In this dissertation, we design and implement a PID control based approach for adaptive video streaming in cellular networks. We start with analyzing existing state-of-the-art video streaming approaches from a control-theoretic point of view, and identifying their limitations. Motivated by the wide adoption and success of PID control in feedback systems, we develop a PID based strategy that optimizes QoE in an online manner using both buffer occupancy and estimated link bandwidth at the client. Evaluation using a large set of real-world cellular traces demonstrates that our solution outperforms existing schemes in a wide range of settings. Our approach does not require accurate link bandwidth prediction. On the other hand, its performance can be further improved with accurate link bandwidth prediction using LinkForecast.

\section{Contribution of This Dissertation}

The contributions of this dissertation are as follows.

\begin{itemize}
\item We investigate various information from the radio interface of a mobile device, and identify several key parameters that have strong correlation with cellular link capacity. Our study significantly expands the scope of existing studies~\cite{Schulman:2010:BPA:1859995.1860006,Chakraborty:2013:CCB:2500423.2500447,soroush2013turning} that only focus on one or two types of information.

\item Based on the key parameters that identified, we develop a machine learning based prediction framework, \emph{LinkForecast}, that uses the identified radio information to predict link bandwidth in real-time. %Compared to existing studies that rely on transport layer information (e.g.,~\cite{Jiang:2012:TBN:2398776.2398810, Xu:2013:Proteus, Winstein:2013:SFA:2482626.2482670}), our approach of using radio-layer information for prediction has the advantage that it is applicable even in the absence of any data to mobile devices. And
    Evaluations demonstrate that our prediction is highly accurate: even at the time granularity of one second, the average relative errors are 4.7\% and 6.9\% under static and walking scenarios, and are 4.3\% and 9.3\% under local and highway driving scenarios, respectively. The relative errors are even lower for larger time granularity. %For instance, the average relative error is reduced to 1.4\% and 2.2\% under the two latter mobile scenarios when the time granularity is 4 seconds.

\item We design a new congestion control protocol for LTE networks. To the best of our knowledge, this is the first transport protocol that directly utilizes real-time link bandwidth prediction. Extensive evaluation using large-scale traces from a commercial LTE network demonstrates that our protocol achieves both high throughput and low delay. It significantly outperforms traditional TCP protocols in both link utilization and latency. %Compared with Sprout~\cite{Winstein:2013:SFA:2482626.2482670}, a recent state-of-the-art protocol that is designed for cellular networks, our protocol achieves similar or better performance while our protocol is much simpler and does not require long training period.
     %It outperforms widely used TCP variants as well as a recent end-to-end protocol that is designed for cellular networks~\cite{Winstein:2013:SFA:2482626.2482670}. For instance, in evaluations on traces from a commercial LTE network, our scheme, compared with the Linux default TCP Cubic, reduces the average delay in half, while achieves an even higher throughput.
\item We examine existing state-of-the-art video streaming adaptation schemes from a control-theoretic point of view, and identify their limitations. Motivated by the wide adoption and success of PID control in feedback systems, we develop a PID based adaptation algorithm that optimizes QoE in an online manner using both buffer occupancy and link bandwidth information at the client. Evaluations using a large set of real-world cellular traces demonstrate that our solution outperforms existing schemes under various network conditions and different user's QoE preferences. While our approach does not require a very accurate link bandwidth prediction, its performance is further improved when using the accurate link bandwidth predictions from LinkForecast.
\end{itemize}


\section{Dissertation Roadmap}

The remainder of this dissertation is organized as follows.

In Chapter~\ref{chapter:linkforecast}, we describe our work on predicting cellular link bandwidth using lower-layer information.
%In Section~\ref{sec:lte_basics}, we describe LTE basics including LTE network architecture and scheduling process of eNodeB.
In Section~\ref{sec_data_collection} and Section~\ref{sec:dataset}, we describe the data collection methodology and the data set used throughout this dissertation, respectively. In Section~\ref{sec:correlation}, we investigates the correlation between various radio layer information and cellular link bandwidth. In Section~\ref{sec:prediction} we presents the design and performance of our link bandwidth prediction framework LinkForecast. And in Section~\ref{sec:discuss}, we discuss a couple of practical issues.

In Chapter~\ref{chapter:ltp}, we present our work on designing a new transport protocol LTP that utilizes link bandwidth prediction from LinkForecast.
In Section~\ref{sec:lte_design}, we describe the design of LTP. And in Section~\ref{simu}, we evaluate the performance of LTP under various scenarios.

In Chapter~\ref{chapter:pid}, we design a PID-based control algorithm for adaptive video streaming over cellular networks.
In Section~\ref{sec:pid_intro} we introduce the background of adaptive video streaming and PID control.
In Section~\ref{sec:streaming_background}, we describe the related work on video streaming.
In Section~\ref{sec:control_model} we formulate the problem, examine existing solutions from a control-theoretic point of view, and propose our PID-based video streaming adaptation algorithm. In Section~\ref{sec:pid_eval}, we evaluate the performance the proposed solution under a wide range of settings.

Finally in Chapter~\ref{chapter:conclusion} we conclude the dissertation and present future directions.

\fi 


==> macros.tex <==
%%%% Add any personal macros here.

==> pid.tex <==


%\input{pid/intro}
%\input{pid/related}




==> preamble.tex <==
%There are portions of this file which are editable, and portions which should not be adjusted.  I've clearly labeled the section where your customizations should be written.

%%%%%%%%%%%%%%%%%%%%
%% Do not edit!!! %%
%%%%%%%%%%%%%%%%%%%%
\usepackage{
	amsmath,
	amsthm,
	amssymb,
	fancyhdr,
	setspace,
}
\usepackage[
	paper=letterpaper,
	left=1.5in,
	top=1in,
	bottom=1in,
	right=1in,
	includehead,
	includefoot
]
{geometry}
\usepackage[titles]{tocloft}
\setlength{\cftbeforechapskip}{2ex}
\setlength{\cftbeforesecskip}{0.5ex}
\renewcommand{\cftchapfont}{\bfseries}
\renewcommand{\cftchapaftersnum}{.}
\renewcommand{\cftsecfont}{}
\renewcommand{\cftchappagefont}{\mdseries}
\renewcommand\cftchappresnum{Ch.\,}
\setlength{\cftchapnumwidth}{3.75em}
\usepackage{sectsty}
\allsectionsfont{\singlespacing}
\pagestyle{fancy}
\rhead{\thepage}
\cfoot{}
\lhead{}
\chead{}
\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}

%%%%%%%%%%%%%%%%%%%%
%%%%% Editable %%%%%
%%%%%%%%%%%%%%%%%%%%

%\usepackage{<add your packages>}

\usepackage[center,small,sc]{caption}
\usepackage{graphics}
\usepackage{epsfig}
\usepackage{hyperref}
\usepackage{multirow}

\input{bing-command}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\theoremstyle{definition}
\newtheorem{dfn}[thm]{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem{remark}[thm]{Remark}
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}

%%%%%%%%%%%%%%%%%%%%
%% Do not edit!!! %%
%%%%%%%%%%%%%%%%%%%%
\input{macros.tex}
\doublespacing 

==> prediction.tex <==
\section{Analysis of Radio Information}
\label{sec:correlation}


We analyze all the available LTE related physical and MAC layer information provided by QxDM. In the following, we describe a set of parameters that are identified to be correlated with cellular link bandwidth. For each parameter, we first describe the intuition why the correlation might be significant, and then present quantitative measurement results.
%Since the correlation may depend on time, location, and mobility, we analyze the traces in each category listed in Table~\ref{table_data1}.
%four broad categories:  static, walking, local driving and highway driving, as well as sub-categories depending on time and location.

We use multiple time granularity (i.e., time unit $\Delta$ is 1, 2, 4, or 10 seconds) when analyzing the correlation between radio information and link bandwidth. We only present the results based on the time granularity of one second; the results for other time granularity are similar.
For clarity, we first present the results based on the data collected from Samsung Note 3 in AT\&T network (see Table~\ref{table_data1}). Then we briefly describe the results in other settings.



%in certain cases. Time granularity 1 second, 4 seconds. In this section, we present when a lower-layer information is correlated with link bandwidth and the extent of correlation.
%Sampling rate: CQI: 320ms, RSRQ: 160ms, TBS: 20ms, BLER: 20ms.


\subsection{Signal Strength}
%One of the most intuitive parameters related to cellular link bandwidth is signal strength.
Three types of signal strength information are available from the radio interface: RSSI (Received Signal Strength Indicator), RSRP (Reference Signal Received Power), and RSRQ (Reference Signal Received Quality). RSSI represents the \emph{total} power a UE observes across the whole band, including the main signal and co-channel non-serving cell signal, adjacent channel interference and the noise within the specified band.
%Therefore RSSI alone is not a good indicator of achievable network performance, i.e., high RSSI does not guarantee high throughput/low delay.
RSRP is the linear average (in watts) of the downlink reference signals across the channel bandwidth. It measures the absolute power of the reference signal. RSRQ is defined as $(N \cdot \mbox{RSRP})/\mbox{RSSI}$, where $N$ is the number of resource blocks over the measurement bandwidth. In other words, RSRQ indicates what the portion of pure reference signal power is over the whole E-UTRAN power received by the UE.

%present the correlation of RSSI, RSRQ, and RSRP with link bandwidth in various scenarios:
%RSRQ plays a more important role in moving scenarios.
%For static case, when the network is less congested (night), RSRQ plays a less important role, while RSRP is more important.

%%wb, 3/9/2015
%%RSRP: scatter plot for highway driving; correlation for highway driving (using all the traces)
%RSRP-highway-scatter.pdf
%RSRQ-highway-scatter.pdf
%RSRP-RSRQ-highway-corr.pdf

%RSRP-office-idle-scatter.pdf
%RSRQ-office-idle-scatter.pdf
%RSRP-RSRQ-idle-corr.pdf

%RSRP-office-busy-scatter.pdf
%RSRQ-office-busy-scatter.pdf
%RSRP-RSRQ-busy-corr.pdf

%%interesting observations:
%%correlations for RSRP and RSPQ are similar (differ from observations in LoadSense)
%%observe correlation in all cases except for office idle for RSRQ; more mobile scenarios have larger correlation

%\tydubfigsingle{fig/fig/RSRP-highway-scatter}{}{fig/fig/RSRQ-highway-scatter}{}{(a) Scatter plot of link bandwidth and RSRQ. (b) Scatter plot of link bandwidth and RSRP. Both based on data in highway-driving scenario.}{RSRP-RSRQ-scatter}

\tydubfigsingle{fig/fig/RSRP-highway-scatter}{RSRP}{fig/fig/RSRQ-highway-scatter}{RSRQ}{(a) Scatter plot of signal strength and link bandwidth for highway-driving scenario.}{RSRP-RSRQ-scatter}

%\singlefig{fig/fig/RSRP-RSRQ-highway-corr}{Correlation coefficient between signal strength (RSRP or RSRQ) and link bandwidth for highway-driving scenario.}{RSRP-RSRQ-corr}

\tydubfigsingle{fig/fig/RSRP-corr}{RSRP}{fig/fig/RSRQ-corr}{RSRQ}{Correlation coefficient between signal strength (RSRP and RSRQ) and link bandwidth for various scenarios.}{RSRP-RSRQ-corr}

%only in office idle setting, observe almost no correlation between RSRQ and link bandwidth (maybe because no interference)
\tydubfigsingle{fig/fig/RSRP-RSRQ-busy-corr}{daytime}{fig/fig/RSRP-RSRQ-idle-corr}{night time}{Correlation coefficient between signal strength (RSRP or RSRQ) and link bandwidth for static campus scenario.}{RSRP-RSRQ-office-corr}

Since RSSI does not measure specifically the link between a UE and eNodeB, we focus on the other two types of signal strength information, namely, RSRP and RSPQ. We observe that RSRP is correlated with link bandwidth in all cases. Fig.~\ref{fig:RSRP-RSRQ-scatter}(a) is a scatter plot of RSRP and link bandwidth under the highway driving scenario, where each point represents the average bandwidth over one second and the corresponding average RSRP over that second.  We observe that when RSRP is very low, link bandwidth tends to be low as well (see lower left corner); similarly, when RSRP is very high, link bandwidth tends to be high as well (see upper right corner). Similar correlation is observed between RSRQ and link bandwidth (see scatter plot in Fig.~\ref{fig:RSRP-RSRQ-scatter}(b)).

Fig.~\ref{fig:RSRP-RSRQ-corr} plots cross correlation between signal strength (RSRP or RSRQ) and link bandwidth under various scenarios. Specifically, for each scenario, we obtain two time series, $\{b_i\}$ and $\{r_i\}$, where $b_i$ and $r_i$ are respectively the average link bandwidth and signal strength (RSRP or RSRQ) during the $i$th second. We explore the cross correlation with lag $l$, i.e., between $b_{i+l}$ and $r_i$, where $l=0, 1, \ldots, 30$ seconds. We observe that the correlation is significant even at the lag of tens of seconds except for the walking scenario (where the correlation is only significant at the lag of a few seconds). In general, we observe that the correlation between RSRP and link bandwidth is comparable to that between RSRQ and link bandwidth. This observation differs from the observation in~\cite{Chakraborty:2013:CCB:2500423.2500447}, which shows that RSRQ is more correlated with link bandwidth than RSRP. The difference might be because the results in~\cite{Chakraborty:2013:CCB:2500423.2500447} are from a more congested 3G network.
We also observe that the correlation between signal strength (RSRP or RSRQ) and link bandwidth is larger for high mobility scenarios (local and highway driving) compared to low mobility scenarios (static and walking).

%Namely, the correlation is lower in less mobile scenarios.
Fig.~\ref{fig:RSRP-RSRQ-office-corr} plots the correlation coefficients between signal strength and link bandwidth in a static setting in a university campus. Figures~\ref{fig:RSRP-RSRQ-office-corr}(a) and (b) differ in that one is collected during daytime, while the other is collected in night time, both of a total duration of 2800 seconds. Interestingly, we observe that the correlation between RSRQ and link bandwidth is close to zero. This is the only scenario where RSRQ is not correlated with link bandwidth. Inspecting the trace, we think this might be because during night time, RSRQ is fairly stable while link bandwidth fluctuates over time.
%The exact reason is not clear. On the other hand,
%While we do not know exactly the reason for the low correlation, it demonstrates that the correlation between signal strength and link bandwidth indeed depends on time, location and mobility.


\subsection{Channel Quality Indicator (CQI)}
As the name implies, CQI is an indicator carrying the information on the quality of the communication channel.
It is a 4-bit integer (i.e., the value is between 0 and 15), and is determined by a UE~\cite{3gppts36213}. LTE specification does not specify how a UE calculates CQI.
In general, a UE takes into account multiple factors (e.g., the number of antennas, signal-to-interference-noise-ratio (SINR), the capability of its radio) when calculating CQI.
The calculated CQI is reported to the eNodeB, which performs downlink scheduling accordingly.
%, to suggest a fast and reliable connection speed.
%CQI reporting plays an important role in eNodeB selecting an proper transmission rate for UE.
%Based on the reported CQI value, eNodeB performs downlink scheduling and link adaptation.

%\tydubfigsingle{fig/cqi}{}{fig/cqi_corr_new}{}{(a) Link bandwidth and CQI versus time. (b) Correlation coefficient between link bandwidth and CQI.}{CQI}

%wb, 3/10/2015, having one scatter plot is sufficient
%\tydubfigsingle{fig/fig/CQI-highway-scatter}{highway driving}{fig/fig/CQI-office-idle-scatter}{static (campus, nighttime)}{Scatter plot of Link bandwidth and CQI.}{CQI-scatter}

%\singlefig{fig/fig/CQI-highway-corr}{Correlation coefficient between CQI and link bandwidth for various scenarios.}{CQI-corr}

\tydubfigsingle{fig/fig/CQI-highway-scatter}{}{fig/fig/CQI-corr}{}{(a) Scatter plot of Link bandwidth and CQI in highway driving scenario. (b) Correlation coefficient between CQI and link bandwidth for various scenarios.}{CQI-overall}

%almost no correlation
%\singlefig{fig/fig/CQI-office-busy-scatter}{Correlation coefficient between CQI and link bandwidth for static (campus, daytime).}{CQI-corr}
%use both scatter plot and correlation curve

%wb, 3/11/2015, merge it with the earlier figure
%\tydubfigsingle{fig/fig/CQI-office-busy-scatter}{}{fig/fig/CQI-office-idle-busy-corr}{}{(a) Scatter plot of Link bandwidth and CQI in static (campus, daytime) scenario. (b) Correlation coefficient between CQI and link bandwidth for static campus daytime and nighttime.}{CQI-office}


%A recent study~\ref{Lu15:CQIC} uses CQI for prediction. {\textbf When static, CQI is not a good indicator.}
%We observe that CQI is correlated with link bandwidth in most cases. As an example, the correlation can be visually observed in the scatter plots in Figures~\ref{fig:CQI-overall}(a) and (b), which are for highway driving and static (campus, nighttime) scenarios. In general, the correlation between CQI and link bandwidth decreases with mobility. Fig.~\ref{fig:CQI-corr}

We observe that CQI is correlated with link bandwidth in most cases. As an example, the correlation can be visually observed in the scatter plots in Fig.~\ref{fig:CQI-overall}(a), which is for highway driving scenario. In general, the correlation between CQI and link bandwidth is the highest under highway driving scenario, and is lower under other scenarios.

Fig.~\ref{fig:CQI-overall}(b) plots the correlation coefficient of CQI and link bandwidth under various scenarios. We find that in one scenario (static on campus during daytime), the correlation between CQI and link bandwidth is very low. For the other cases, the correlation is significant even when the lag is up to a few or tens of seconds.
% (see Fig.~\ref{fig:CQI-office}).


%plots both the CQI and the link bandwidth for a randomly selected ten-minute trace. Furthermore, we study the overall correlation between CQI and link bandwidth for all the traces we collected. Fig.~\ref{fig:CQI}(b) plots the correlation coefficient for varying time window and time lag. We observe a strong correlation between CQI and the link bandwidth. In addition, even at the time lag of five seconds, the correlation is still fairly close to that when the time lag is zero.

%%wb, 3/9/2015
%CQI high for highway driving, reasonably high for local driving
%low for busy case (walking and static); maybe in this case, scheduling plays an important role
%CQI-highway-scatter.pdf
%CQI-highway-corr.pdf

%CQI-office-idle-scatter.pdf
%CQI-office-busy-scatter.pdf
%CQI-office-idle-busy-corr.pdf


%\subsubsection{MCS and Number of RB}
\subsection{Resource Allocation}
\label{sec:mcs}

In LTE networks, time-frequency resources are allocated in units of resource blocks (RBs). A resource block consists of 12 consecutive sub-carriers, or 180 kHz, for the duration of one slot (0.5 ms). The scheduling decision of an eNodeB for a UE includes a specific Modulation and Coding Scheme (MCS) and the number of resource blocks (nRB). The first parameter, MCS index is in the range of 0 to 31. It summarizes the modulation type and the coding rate that are used in the allocated RBs. Typically, a higher MCS index offers a higher spectral efficiency (which translates to a higher potential data rate), but requires a channel with better quality to support it. The second parameter, nRB, determines how many resource blocks are allocated to a UE. With the MCS index and nRB, the Transport Block Size (TBS) can be uniquely determined by looking up the mapping tables defined in 3GPP 36.213~\cite{3gppts36213}.
In general, a higher value of MCS and a larger nRB yield a larger TBS, and thus lead to higher link bandwidth.

%%wb, 3/9/2015
%TBS for all the cases, in scatter plot with linear regression curve
%correlation (all correlations in the same figure)

\tydubfigsingle{fig/fig/TBS/Highway_tbs}{Highway driving}{fig/fig/TBS/Office_new_Idle_tbs}{Static (campus, night time)}{Scatter plot of link bandwidth and CQI. The linear curves represent the results from linear regression.}{TBS-scatter}

\bigsinglefig{fig/fig/TBS/TBS_corr}{Correlation coefficient between TBS and link bandwidth for various scenarios.}{TBS-corr}

We observe that TBS is strongly correlated with link bandwidth in all the cases. In addition, the relationship between $b_i$ and $TBS_i$ is very similar in all the cases, where $b_i$ and $TBS_i$ denote respectively the average link bandwidth and the aggregate TBS in the $i$th second. Fig.~\ref{fig:TBS-scatter} shows the scatter plot between $b_i$ and $TBS_i$ in two very different scenarios, one corresponding to highway driving and the other corresponding to static scenario (on a university campus during night time). Both plots show a strong linear relationship between $b_i$ and $TBS_i$. The linear regression models for the two cases have similar coefficients. Of all the cases, we have $b_i = \alpha TBS_i + \beta$, where $\alpha$ is between $0.0059$ and $0.0070$, and $\beta$ is between 600 and 1500 (which is very small given that $b_i$ can be up to tens thousands of Kbps).

Fig.~\ref{fig:TBS-corr} plots the correlation coefficient between TBS and link bandwidth for various scenarios. We observe very high correlation (above 0.8) when the lag is a few seconds. Even when the lag is tens of seconds, the correlation is still significant.


%%wb, 3/11/2015, concurrently or in pipeline mode???
\subsection{Block Error Rate (BLER)}
Hybrid-ARQ (HARQ) is used in LTE networks to achieve higher efficiency in transmission and error correction. It uses 8 stop-and-wait processes to transmit data. Once a packet is sent from a particular process, the process will be in active state and will not process other packets until it receives an ACK or NACK. If a NACK is received, then a retransmission will be initiated.
If too many retransmissions happen, the eNodeB has to adjust the modulation and coding scheme.
%Although the concurrent processes significantly reduce the round trip time and thus increase link speed, if HARQ is working frequently for error recovery, the throughput will decrease considerably.
Specifically, HARQ Block Error Rate (BLER) is defined as the number of erroneous blocks divided by the total number of blocks that are sent.
The target BLER is typically 10\%~\cite{3gppts36213}. If the actual BLER is larger than 10\% (e.g., due to weak signal strength or interference), the link must be switched to a lower speed, and vice versa.

%%wb, 3/11/2015, the correlation coefficients are fairly small, use scatter plot instead
%\tydubfigsingle{fig/bler}{}{fig/bler_corr_new}{}{(a) Link bandwidth and BLER versus time. (b) Correlation coefficient between link bandwidth and BLER.}{bler}

\tydubfigsingle{fig/bler}{}{fig/fig/BLER_highway}{}{(a) Link bandwidth and BLER versus time. (b) Scatter plot between link bandwidth and BLER (highway driving scenario).}{bler}

Fig.~\ref{fig:bler}(a) plots link bandwidth and BLER over time for a five-minute long trace. We see the BLER is fluctuating around 10\%; when the BLER is high, the link bandwidth is low.
%Fig.~\ref{fig:bler}(b) plots the correlation coefficient between link bandwidth and BLER for varying time window and lag. The correlation coefficient is negative, and indicating strong correlation even when the time lag is two seconds.
Fig.~\ref{fig:bler}(b) is a scatter plot between link bandwidth and BLER under the highway driving scenario. We observe that most of the BLER values are between 0.05 and 0.1. When BLER is above 0.1, the link bandwidth tends to be low. On the other hand, when BLER is below 0.1, the link bandwidth is in a wide range. As a result, the cross correlation between BLER and link bandwidth is not significant (figure omitted).


\subsection{Handover Events}
A handover is performed when a UE moves from the coverage of one cell to the coverage of another cell in the connected state. Unlike the case in UMTS, there are only hard handovers in LTE networks, i.e., a UE cannot communicate with multiple eNodeBs simultaneously. Therefore, there will be a short interruption in service when a handover happens. The impact of the LTE handover procedures on the user experience depends very much on the type of the application that is being used. For instance, a short interruption in a large file downloading may not be even noticeable, while an interruption in a delay-sensitive application (e.g., VoIP, video streaming, interactive online gaming) can be very disruptive. We use the changes in serving cell ID  to detect the handover events.
%For example, a short interruption in service during a long FTP session (e.g., large file downloading) may be tolerable, but an interruption in a latency sensitive application (e.g., VoIP, video streaming, interactive online gaming) may not. To capture handover events, we keep monitoring the serving cell ID. A change in serving cell ID indicates a handover event.

%\tydubfigsingle{fig/handover}{}{fig/handover_corr_new}{}{(a) Link bandwidth and handover events. (b) Correlation coefficient between link bandwidth and handover events.}{handover}

\singlefig{fig/handover}{Link bandwidth and handover events.}{handover}

%\smsinglefig{fig/handover}{Link bandwidth and handover events.}
Fig.~\ref{fig:handover} plots a sample trace of link bandwidth where handover events are marked as red dots. It shows that an instant decrease in bandwidth when handover happens. We represent handover events as a binary time series $\{h_i\}$, where $h_i=1$ if there exists a handover event in the $i$th second and $h_i=0$ otherwise. Again let $\{b_i\}$ represent the average link bandwidth in the $i$th second. Calculating the cross correlation between $\{h_i\}$ and $\{b_i\}$ does not reveal significant correlation in any of the scenarios (the most significant correlation is under highway driving where the correlation under lag 1 is around -0.1). This might be because of the infrequency of handover events.
%Fig.~\ref{fig:handover}(b) plots the correlation coefficient between link bandwidth and handover events. We only plot the results when time lag is 0. The correlation is significant; the large variation is due to the infrequency of handover events.

%\input{ana-uplink}


\subsection{Time Granularity} \label{subsec:granularity}

%The results presented above use time granularity of one second. The results under other granularity (2, 4, and 10 seconds) are consistent with those under one second granularity. We still observe that RSRP, RSRQ, CQI, BLER and handover events are correlated with link bandwidth in various scenarios.

%\iffalse

The results presented above using time granularity of 1 second. The results under other granularity (2, 4, and 10 seconds) are consistent with those under one second granularity. We still observe that RSRP, RSRQ, CQI, TBS, BLER and handover events are correlated with link bandwidth in various scenarios, and TBS has the highest and most consistent correlation across all the scenarios.

Fig.~\ref{fig:TBS-scatter-4s} shows the scatter plot between link bandwidth and TBS in highway driving and static (on a university campus during night time) scenarios. We again observe a strong linear relationship between these two quantities. The linear regression models for the two scenarios (and also other scenarios) have similar coefficients. Compared with the results using one second as granularity (see Fig.~\ref{fig:TBS-scatter}), the points are closer to the linear line because the amount of randomness is lower when using a larger granularity. In addition, the slope of the line is around one fourth of the value under one second granularity since the TBS is the aggregate over 4 seconds (approximately four times as the aggregate over one second).

\tydubfigsingle{fig/fig4s/TBS/Highway_tbs}{Highway driving}{fig/fig4s/TBS/Office_new_Idle_tbs}{Static (campus, night time)}{Scatter plot of link bandwidth and TBS when the time granularity is 4 seconds. The linear curves represent the results from linear regression. }{TBS-scatter-4s}
%\fi

\subsection{Other Phones and Networks}
The analysis above is based on the traces collected from Samsung Note 3 (denoted as Phone 1) in AT\&T network.
In order to understand whether the correlation still holds for different phones, we pick a much older and less powerful Samsung S3 (denoted as Phone 2) on purpose, and collect traces in both static and walking scenarios. While Phone 2 achieves a similar average throughput as Phone 1 (5.3 Mbps versus 5.7 Mbps in static scenario and 7.7 Mbps versus 7.9 Mbps in walking scenario). We observe that Phone 2 in general uses many more resource blocks and slower modulation and coding schemes.
\tydubfigsingle{fig/fig/mcs_phone2}{MCS}{fig/fig/nrb_phone2}{nRB}{Scatter plot of link bandwidth and MCS and nRB of the two phones under static (campus, night time) scenario.}{mcs-scatter-phone2}
Figures~\ref{fig:mcs-scatter-phone2}(a) and (b) show the scatter plots for MCS and nRB, respectively, for the two phones. From the figure, we can observe that Phone 2 uses much lower MCS than Phone 1. In other words, the sending speed for each resource block is much slower than Phone 1. However, in order to compensate for the lower MCS, we also observe that Phone 2 is allocated as many as 50 resource blocks, while Phone 1 gets at most 25. In some sense, eNodeB allocates more resource to Phone 2 to compensate for the inferior radio capability.

\singlefig{fig/fig/tbs_phone2}{Scatter plot of link bandwidth and TBS of the two phones under static (campus, night time) scenario.}{tbs-scatter-phone2}

Fig.~\ref{fig:tbs-scatter-phone2} shows the scatter plot of link bandwidth and TBS for the two phones. As explained earlier, TBS reflects the combined effect of both MCS and nRB. We observe that the two phones actually exhibit a very similar correlation between link bandwidth and TBS. For Phone 2, the correlations between other factors and link bandwidth are similar as those for Phone 1 (figures omitted).

We also evaluate the correlation results for other phones and Verizon network. 
Overall, the results exhibit very similar trends. For instance, when using Samsung S5 on Verizon network, at lag 1, the correlation coefficients of RSRP and link bandwidth range from 0.42 to 0.60 for various scenarios, for RSRQ and CQI, the correlation coefficients range from 0.31 to 0.52, and 0.32 to 0.61, respectively.


==> related.tex <==
\section{Related Work} \label{sec:related}
\label{chapter:related}
%prediction based paper (PROTEUS, mobicom paper);

%%need to add CQIC paper and Gil's paper
Bandwidth estimation has been studied extensively in wired networks (e.g.,~\cite{downey99using,Dovrolis04:dispersion}) and wireless LANs (e.g.,~\cite{Lakshminarayanan04:bandwidth,Li08:Wbest}). The study in~\cite{Koutsonikolas09:feasibility} demonstrates that existing bandwidth estimation techniques for wired networks and wireless LANs are not effective in cellular networks. Xu et al.~\cite{Xu:2013:Proteus} develop a system interface called PROTEUS that forecasts future network performance (throughput, loss, and one-way delay) based on current measurements, and integrate PROTEUS with real-time communication applications. Winstein et al.~\cite{Winstein:2013:SFA:2482626.2482670} use packet inter-arrival time to infer link bandwidth and further determines the number of packets that can be transmitted. The techniques in~\cite{Xu:2013:Proteus,Winstein:2013:SFA:2482626.2482670} rely on network metrics. %Hence they are only applicable when there exists traffic on a UE, and the aggregate rate of the traffic matches the link bandwidth.

The studies in~\cite{Schulman:2010:BPA:1859995.1860006,Chakraborty:2013:CCB:2500423.2500447,soroush2013turning,Margolies14:mobility,Lu15:CQIC} use low-layer radio information to predict link bandwidth. Schulman et al. find that signal strength (RSSI) is correlated with link bitrate and power consumption, and propose an energy-aware scheduling algorithm for different workloads~\cite{Schulman:2010:BPA:1859995.1860006}. Chakraborty et al. develop a SVM (Support Vector Machine) based technique that categorize bandwidth into two classes (high and low bandwidth), and propose a technique for UEs to coordinate cellular background transfer in an efficient manner~\cite{Chakraborty:2013:CCB:2500423.2500447}. Sorous et al. find that signal strength and throughput are correlated to some extent~\cite{soroush2013turning}, and demonstrate that measurement of throughput at a server can be used to reveal user location. Margolies~\cite{Margolies14:mobility} et al. generate throughput prediction for a mobile device based on the observation that the signal quality of a device is remarkably reproducible for multiple drives on the same path.
While our work also uses radio information, it differs from the above studies in that it investigates an extensive set of radio-layer information, and constructs a prediction model that predicts in realtime link bandwidth in LTE networks.

The work that is closest to ours is~\cite{Lu15:CQIC}. Our study is independent and in parallel to~\cite{Lu15:CQIC}, and differs from~\cite{Lu15:CQIC} in several important aspects. The study in~\cite{Lu15:CQIC} uses CQI and DRX (discontinuous transmission) ratio to predict link bandwidth in HSPA+ networks. The prediction is by looking up a mapping table at a base station. Since the mapping table is vendor implementation dependent, the authors propose to use crowdsourcing to obtain the mapping table at each base station. Our goal is to identify a comprehensive set of radio information that can be used to provides highly accurate link bandwidth prediction, and then use it as an upper bound to identify a small set of information that can achieve most of the gains in LTE networks. We use machine learning techniques for prediction and demonstrate that our approach is not sensitive to training data. In addition, using an extensive data set, we quantify the correlation between various radio information and link bandwidth under different scenarios.

%the ``best" prediction
%%wb, 3/10/2015, not plan to include LTP in this submission
\iffalse
The study on transport protocols is extensive.
We only briefly review several recent studies on transport protocols in cellular networks that are most related to ours.
Jiang et al.~\cite{Jiang:2012:TBN:2398776.2398810} investigate the ``bufferbloat'' problem (i.e., performance degradation caused by oversized buffers inside the network) and proposed an RTT-based congestion window adjustment scheme to reduce latency.
%Our work differs from the above studies in that we investigate an extensive set of radio parameters, and construct a prediction model that is able to adapt to the rapidly changing link conditions in real time.
Winstein et al.~\cite{Winstein:2013:SFA:2482626.2482670} developed Sprout, a transport protocol that models packet arrivals as Poisson process, and use the model to forecast the amount of data that can
be sent by the sender. In \cite{Winstein13:Remy,Winstein14:Remy}, the authors propose Remy, a computer program that create TCP congestion-control algorithms that can be used in a wide range of settings (including cellular networks), and used the Remy automatic protocol-design program as a tool to investigate the ``learnability'' of the Internet congestion-control problem. Our study propose a transport protocol that uses link bandwidth prediction from radio information directly, as a case study to demonstrate the benefit of LinkForecast.
\fi

Several studies investigated the relationship between radio status and performance at an end device. Liu et al. studied the interplay between wireless channels and applications in CDMA networks~\cite{Liu:2008:ENI:1409944.1409969}.
To capture the radio information, Vallina-Rodriguez et al. implemented a tool named RilAnalyzer~\cite{Vallina-Rodriguez:2013:RCM:2504730.2504764}, which can record the radio connection status and application behaviors. While our study also considers radio information and higher-layer performance, it differs in scope from them.


\iffalse
The study on transport protocols is extensive.
We only briefly review several recent studies on transport protocols in cellular networks that are most related to ours.
Jiang et al.~\cite{Jiang:2012:TBN:2398776.2398810} investigated the ``bufferbloat'' problem (i.e., performance degradation caused by oversized buffers inside the network) and proposed an RTT-based congestion window adjustment scheme to reduce latency.
Xu et al.~\cite{Xu:2013:Proteus} developed a system interface called PROTEUS that forecasts future network performance (such as throughput, loss, and one-way delay) based on current measurements, and integrate PROTEUS with real-time communication applications. Winstein et al.~\cite{Winstein:2013:SFA:2482626.2482670} developed Sprout, a transport protocol that models packet arrivals as Poisson process, and use the model to forecast the amount of data that can
be sent by the sender. Our study differs from the above schemes in that we use information collected from the radio interface, not from higher layers, to predict link performance. In addition, our protocol utilizes the predicted link performance directly.

Several studies investigated the relationship between radio status and performance at an end device~\cite{Schulman:2010:BPA:1859995.1860006, Chakraborty:2013:CCB:2500423.2500447, soroush2013turning, Liu:2008:ENI:1409944.1409969}. They however did not provide a fine-grained, real-time solution for link performance prediction or congestion control.
Schulman et al. suggested to communicate when the signal (RSSI) is strong~\cite{Schulman:2010:BPA:1859995.1860006}. Chakraborty et al. proposed to defer the background transfer when the cellular load is below certain thresholds~\cite{Chakraborty:2013:CCB:2500423.2500447}. Sorous et al. found that signal strength and throughput are correlated to some extent~\cite{soroush2013turning}. And Liu et al. studied the interplay between wireless channels and applications in CDMA networks~\cite{Liu:2008:ENI:1409944.1409969}.
To capture the radio information, Vallina-Rodriguez et al. implemented a tool named RilAnalyzer~\cite{Vallina-Rodriguez:2013:RCM:2504730.2504764}, which can record the radio connection status and application behaviors.
Our work differs from the above studies in that we investigate an extensive set of radio parameters, and construct a prediction model that is able to adapt to the rapidly changing link conditions in real time.
\fi

